Learning Software Bug Reports: A Systematic Literature Review

The recent advancement of artificial intelligence, especially machine learning (ML), has significantly impacted software engineering research, including bug report analysis. ML aims to automate the understanding, extraction, and correlation of information from bug reports. Despite its growing importance, there has been no comprehensive review in this area. In this paper, we present a systematic literature review covering 1,825 papers, selecting 204 for detailed analysis. We derive seven key findings: 1) Extensive use of CNN, LSTM, and $k$NN for bug report analysis, with advanced models like BERT underutilized due to their complexity. 2) Word2Vec and TF-IDF are popular for feature representation, with a rise in deep learning approaches. 3) Stop word removal is the most common preprocessing, with structural methods rising after 2020. 4) Eclipse and Mozilla are the most frequently evaluated software projects. 5) Bug categorization is the most common task, followed by bug localization and severity prediction. 6) There is increasing attention on specific bugs like non-functional and performance bugs. 7) Common evaluation metrics are F1-score, Recall, Precision, and Accuracy, with $k$-fold cross-validation preferred for model evaluation. 8) Many studies lack robust statistical tests. We also identify six promising future research directions to provide useful insights for practitioners.

==> algo/mnal-learning.tex <==
\begin{algorithm}[t!]
	\DontPrintSemicolon
	%\footnotesize
	
	\caption{Pseudo code for the learning in \approach}
	\label{alg:mnal}
	\KwIn{A pool of unlabeled reports $\mathbfcal{D}_u$; a pool of all labelled reports $\mathbfcal{D}_l$ and a pre-trained neural language model $\mathbfcal{M}$}
     %\KwOut{The $k$ unlabeled reports to be queried $\mathbfcal{D}_{q}$}

   %$\mathbfcal{D}_l=\emptyset$ \tcc*[h]{\textcolor{blue}{the pool of all labelled reports.}}\\
   \For{$t \in \{0,...,T\}$}
   {
        \If{$\mathbfcal{M}=\emptyset$ or $\mathbfcal{D}_l$ has been updated since last timestep} 
        {
          $\mathbfcal{M}\leftarrow$ update a neural language model using $\mathbfcal{D}_l$\\
          %$\mathbfcal{D}_l=\mathbfcal{D}_i$\\
        }
        $\mathbfcal{D}_q\leftarrow$\textsc{EUSampling}($\mathbfcal{M}$,$\mathbfcal{D}_u$) \tcc*[h]{\textcolor{blue}{effort-aware uncertainty sampling the top $k$ unlabeled reports.}}\\
        $\mathbfcal{D}_q\leftarrow$ the developers label all the queried reports\\

        $\mathbfcal{D}_u=$ remove all reports in $\mathbfcal{D}_q$ from $\mathbfcal{D}_u$\\
        $\mathbfcal{D}_p\leftarrow$ \textsc{pseudoLabeling}($\mathbfcal{D}_l$,$\mathbfcal{D}_q$,$\mathbfcal{D}_u$) \tcc*[h]{\textcolor{blue}{pseudo-labeling additional $k$ unlabeled reports.}}\\
        $\mathbfcal{D}_u=$ remove all reports in $\mathbfcal{D}_p$ from $\mathbfcal{D}_u$\\
        $\mathbfcal{D}_l$ = $\mathbfcal{D}_l \cup \mathbfcal{D}_q \cup \mathbfcal{D}_p$\\
        update $\mathbfcal{M}$ with $\mathbfcal{D}_l$
   }

    

   % \Return $\mathbfcal{D}_{q}$\\
	
\end{algorithm}

==> algo/pseudo-label.tex <==
\begin{algorithm}[t!]
	\DontPrintSemicolon
	%\footnotesize
	
	\caption{\textsc{pseudoLabeling} function}
	\label{alg:pseudo}
	\KwIn{Historically labeled reports $\mathbfcal{D}_{l}$; the set of newly human-labeled reports $\mathbfcal{D}_q$; all remaining unlabeled reports $\mathbfcal{D}_u$}
     \KwOut{The set of pseudo-labeled reports $\mathbfcal{D}_{p}$ for further consolidating the neural language model}

    %$\mathbfcal{D}_{l}\leftarrow \mathbfcal{D}_{l} \cup \mathbfcal{D}_q$\\
   $\mathbfcal{M}\leftarrow$ update an intermediate version of the neural language model $\mathbfcal{M}$ using all labeled reports so far $\mathbfcal{D}_{l}\cup \mathbfcal{D}_q$\\
   \For{$\forall r_{i} \in \mathbfcal{D}_q$}
   {
        $\mathbfcal{D'}_q\leftarrow \langle r_{i},\mathbf{\overline{v}_i} \rangle =$ get embedding vector $\mathbf{\overline{v}_i}$ when predicting $r_{i}$ using $\mathbfcal{M}$\\
   }

      \For{$\forall r_{j} \in \mathbfcal{D}_u$}
   {
        $\mathbfcal{D'}_u\leftarrow \langle r_{j},\mathbf{\overline{v}_j} \rangle =$ get embedding vector $\mathbf{\overline{v}_j}$ when predicting $r_{j}$ using $\mathbfcal{M}$\\
   }
  % $\mathbfcal{T} = \mathbfcal{L}$\\
    \For{$\forall \langle r_{i},\mathbf{\overline{v}_i} \rangle  \in \mathbfcal{D'}_q$}   
    {
         $d_s=-1$\\
         $r_s=\emptyset$\\
         \For{$\forall \langle r_{j},\mathbf{\overline{v}_j} \rangle \in \mathbfcal{D'}_u$}    
         {
             $d_{ij}=$ calculate the 2-norm distance between $\mathbf{\overline{v}_i}$ and $\mathbf{\overline{v}_j}$\\
             \If{$d_s=-1$ or $d_{ij}<d_s$} 
             {
                $r_s = r_j$\\
                $d_s = d_{ij}$\\
             }
             
         }
          $\mathbfcal{D}_{p}\leftarrow r_s$ with the label of $r_i$\\
         %$\mathbfcal{T}\leftarrow r_s$\\
    }
	
	
	
    

    \Return $\mathbfcal{D}_{p}$\\
	
\end{algorithm}

==> algo/sampling.tex <==
\begin{algorithm}[t!]
	\DontPrintSemicolon
	%\footnotesize
	
	\caption{\textsc{EUSampling} function}
	\label{alg:sampling}
	\KwIn{All remaining unlabeled reports $\mathbfcal{D}_u$; the current neural language model $\mathbfcal{M}$}
     \KwOut{The $k$ unlabeled reports to be queried $\mathbfcal{D}_{q}$}

   \For{$\forall r_{i} \in \mathbfcal{D}_u$}
   {
        $s_i$ = get the effort-accuracy score of $r_{i}$ using $\mathbfcal{M}$ and normalization via Equation~\ref{eq:unc}-\ref{eq:score}\\
        \If{$|\mathbfcal{D}_q| < k$ or $s_i >$ the score of the at least one entry of $\mathbfcal{D}_q$}    
        {
             \If{$|\mathbfcal{D}_q| = k$} {
               remove the last entry of $\mathbfcal{D}_q$\\
              } 
              $\mathbfcal{D}_q\leftarrow r_i$\\
            sort $\mathbfcal{D}_q$ descendingly\\
        }
       
   }

    

    \Return $\mathbfcal{D}_{q}$\\
	
\end{algorithm}

==> sec/exp.tex <==


\section{Experimental Setup}
\label{sec:exp}

In this section, we elaborate on the details of our experiment settings.

\subsection{Research Questions}
The research questions we aim to answer in this study are:
\begin{itemize}
     \item \textbf{RQ1:} How effective is the effort-aware uncertainty sampling?
     \item \textbf{RQ2:} How useful is the pseudo-labeling?
     \item \textbf{RQ3:} To what extent can \approach~improve an arbitrary neural language model?
     \item \textbf{RQ4:} How effective is \approach~against the state-of-the-art approaches for identifying bug reports?
     \item \textbf{RQ5:} What do the human developers think about \approach~in terms of the effort reduction for labeling reports?
\end{itemize}


We explore \textbf{RQ1} to assess the effectiveness and implication of querying unlabeled reports that are both good at improving accuracy and require a reasonable amount of effort to label. In \textbf{RQ2}, we ask how pseudo-labeled reports, which leverage the unique embedding of a neural language model, can complement the prediction performance in an active learning setting. Both \textbf{RQ1} and \textbf{RQ2} help to confirm the usefulness of the mutualistic relation in \approach. Since the design of \approach~is agnostic to the underlying neural language model, we examine \textbf{RQ3} to understand how well it can improve a neural language model compared with the case where the model is trained with data without any sophisticated sampling and pseudo-labeling. To verify the effectiveness of \approach, in \textbf{RQ4}, we compare \approach~against four state-of-the-art active learning approaches for bug report identification, hence confirming the benefit of neural active learning. Finally, in \textbf{RQ5}, we conduct a qualitative study with human involvement to understand the true usefulness of \approach.


%In \textbf{RQ2}, we inquire whether we can enhance the method by seamlessly integrating the pseudo-labeling technique into each step of the effort-aware active learning process. To investigate this, we compare the performance metrics of the effort-aware method when pseudo-labeling is integrated and when it is not, as part of our analysis in \textbf{RQ2}. In \textbf{RQ3}, we conduct an agnostic experiment to assess the adaptability of \approach when using alternative BERT-like models. Specifically, we compare passive learning with \approach that has been configured with different BERT-like models to determine if substantial performance enhancements and reductions in annotation effort are still achievable. To verify the effectiveness of \approach, in \textbf{RQ4}, we compare \approach against four state-of-the-art (SOTA) active learning strategies in bug report identification from the literature, as shown in Section~\ref{sec:rq4}. Finally, in \textbf{RQ5}, we conducted a simulation experiment that emulates real-world application. We invited ten computer science students to annotate 300 reports each, randomly selected into control (passive learning) and experimental (effort-aware strategy using \approach) groups, with metrics such as reading and identification difficulty scores, annotation time, and potential monetary costs.

\subsection{Datasets}

We use the datasets from NLBSE'23\footnote{https://nlbse2023.github.io/tools/}~\cite{nlbse2023}, which is one of the most comprehensive collections of datasets about repository reports to date. In particular, NLBSE'23 contains many smaller datasets and it documents the data in a more structured manner. It is chosen for our evaluation because of its following unique benefits:

\begin{itemize}
    \item \textbf{Large Volume:} The collection of datasets is of a large volume, containing a total of 1,275,881 labeled reports. A detailed breakdown reveals that 670,951 reports, accounting for 52.6\% of the datasets, are bug reports. The remaining 604,930 reports are non-bug reports. Such a near-balanced distribution provides a robust foundation for training and evaluating \approach, ensuring that neither class is underrepresented.
    \item \textbf{Cross-Project :} The datasets contain reports collected from different software projects (over 127,000)\footnote{https://tinyurl.com/mr3h4my7}, which might be of different domains from GitHub. This renders rigorous evaluation of the ability for using \approach~on different projects plausible, which is an important property for neural language model-based approaches.
    \item \textbf{Diverse Report Formats:} The collected reports are of diverse formats and types, ranging from simple interface glitches to complex backend anomalies. The textual descriptions in these reports vary in length and complexity, with some providing detailed steps to reproduce the issue, while others offer a brief overview. This diversity in content and context makes the datasets particularly challenging and, at the same time, an ideal ground for testing the robustness of \approach.
\end{itemize}


%. It is originally for multi-label issue classification tasks. However, for the purpose of our study, we transformed this dataset into a binary classification set, focusing on bug report identification. This transformation involved categorizing reports into two primary classes: bug reports and non-bug reports.

% volumn
% cross project.
% diverse report format.

 

For all experiments, we evaluate the approaches over all data from the datasets, i.e., all of the reports are part of the set of unlabeled reports, thereby we intentionally hide their true labels from the learning approaches. At every timestep, the query size is $k$, meaning that there will be $k$ new reports to be labeled by the human for training. As will be discussed in Section~\ref{sec:diff-k}, we examine different values of $k$. The number of initially labeled reports for \approach~to trigger a cold start of training is also $k$. 

%use the For the purpose of evaluating our method's performance, we extracted a subset of 5,000 reports from the original test set provided by NLBSE2023. This test set offers a diverse range of reports, ensuring a comprehensive assessment of our approach.



\subsection{Experiment Preparation}
We perform some necessary processes and setups to prepare the experiments for \approach~and all other approaches compared:

\begin{itemize}


\item \textbf{Data Preprocessing:} All reports are preprocessed following the steps below:
\begin{enumerate}
    \item  \textit{Symbols Removal:} HTML tags and punctuation marks that appear in the reports are also removed.
    \item  \textit{Stop Words Removal:} Stop words, such as \texttt{\textcolor{blue}{``the''}} and \texttt{\textcolor{blue}{``is''}}, are removed. They appear frequently in natural language but with little contribution to semantic meaning.
    \item \textit{Case Conversion:} All upper case texts are converted into lower case ones.
\end{enumerate}

\item \textbf{Data Splitting:} For training/updating the neural language model or machine learning model (as in the state-of-the-art approaches), we adopt an 80/20 training/validation split when learning each set of $k$ reports. This ensures that the model is trained on a substantial amount of data while also having a separate set for hyperparameter tuning and validation. For testing, we uniformly sample 5,000 reports (with the true labels) from the datasets based on their project, type, length, \textit{etc}; these are excluded from the unlabeled report from the beginning.

%5,000 reports were randomly extracted beforehand solely for the purpose of evaluation/testing for all timesteps and they are unseen by all the approaches during learning.

\item \textbf{Query Size:} To examine different cases of labeling the reports in the process of active learning, we run experiments on three different query sizes, i.e., $k=300$, $k=500$, and $k=700$.

%\item \textbf{Number of Timesteps:} To thoroughly evaluate \approach~while keeping the overhead manageable, we run 10 timesteps and examine the results of each. 

%A fixed set of 5000 samples is reserved exclusively for testing. This ensures that our model's performance is evaluated on unseen data, providing a realistic assessment of its generalization capabilities.

\item \textbf{Human Involvement:} From \textbf{RQ1} to \textbf{RQ4}, we emulate human involvement by assigning the selected reports the true labels from the datasets. For \textbf{RQ5}, we use the judgments given by the human practitioners as the true labels.

\item \textbf{Number of Timesteps and Repetitions:} To emulate a realistic setting, we conduct 10 timesteps for active learning considering the balance between data sufficiency and the time it takes to run the experiment. The initial set of labeled reports for training is selected at random. To account for variability and ensure the robustness of our results, we repeat the entire experiment 10 times with different seeds, wherein each repeat would have different training/updating and testing splits.

\item \textbf{Model and the Parameters:} For the neural language model in \approach, we adopt BERT~\cite{DBLP:conf/naacl/DevlinCLT19} by default, which is pre-trained on Wikipedia data, since it is the most standard and simple one for natural language processing. Such a model will be fine-tuned incrementally with $k$ samples from our downstream task of bug report identification. However, it can be easily replaced with more sophisticated natural language models such as RoBERTa~\cite{DBLP:journals/corr/abs-1907-11692}. We have also evaluated \approach~with different neural language models to confirm its model-agnostic nature (see Section~\ref{sec:rq3}). The hyperparameter settings of those models are either default or tuned to fit the scale of our experiment infrastructure, e.g., for BERT, we use $18$ epochs, $32$ batch size, learning rate of $3 \times 10^{-5}$ and Epsilon factor of $10^{-8}$. For the hyperparameters of other approaches we compared, we set the same values as what was used in their corresponding work.


% \item \textbf{Implementation Details: }All experiments are implemented using Python 3.10. We leverage the APIs from PyTorch and Transformers to build and train our models.

% \item \textbf{Hardware Specifications: }Our experiments run on a high-performance machine equipped with an AMD EPYC 7742 (Rome) 2.25 GHz 64-core CPU. For GPU acceleration, we utilize an NVIDIA A100 with 40 GB RAM, ensuring efficient training and evaluation times.
\end{itemize}

All experiments are implemented using Python 3.10. We leverage the APIs from PyTorch and Transformers to build and train the neural language model in \approach. All experiments are run on a high-performance machine equipped with AMD EPYC 7742 (Rome) 2.25GHz multi-core CPU. For GPU acceleration, we utilize an NVIDIA A100 with 40GB RAM.


\subsection{Metrics}

Since our experiments are both quantitative and qualitative, we design/select different sets of metrics for them.

\subsubsection{Performance (Quantitative)}

We use the following widely used metrics in software repository mining to quantitatively measure the model performance on the testing data at the end of \textit{Timestep} $n$:

\begin{itemize}
 \item \textbf{Precision:} Precision measures the proportion of correctly identified reports among all the reports retrieved, which is defined by:
     \begin{equation}
        Precision = \frac{tp}{tp + fp}
    \end{equation}
 whereby $tp$ and $fp$ are the number of true positive and false positive predictions, respectively. A higher precision signifies that the classification minimizes false positives and predicts information that is highly relevant.

    \item  \textbf{Recall:} Recall measures the ability of a model to identify and retrieve all relevant reports:
     \begin{equation}
        Recall = \frac{tp}{tp + fn}
    \end{equation}
     where $fn$ is the number of false negative predictions. A higher recall score indicates that the model can better reduce false negatives and ensure that a significant portion of relevant data is not overlooked.

    \item \textbf{Accuracy:} Accuracy is a straightforward metric that calculates the ratio of correctly identified reports (both bug and non-bug) to the total number of reports. Formally, it is defined as: 
     \begin{equation}
        Accuracy = \frac{tp+fp}{tp + fp + tn + fn}
    \end{equation}
    whereby $fp$ denotes the number of false positive predictions.
    %In our study, given the near-balanced distribution of bug and non-bug reports, accuracy serves as a reliable indicator of the model's general performance.

    \item \textbf{F1-score:} The F1-score is a harmonic mean of precision and recall, offering a balanced measure between the model's ability to correctly identify bug reports (precision) and its capability to capture all genuine bug reports within the datasets (recall), which is computed as:
     \begin{equation}
        F1\text{ }score = 2 \times \frac{Precision \times Recall}{Precision + Recall}
    \end{equation}   
    In scenarios where the cost of false positives and false negatives is significant, the F1-score becomes an important metric. Given the critical nature of bug report identification, where overlooking genuine bugs or misclassifying non-bug reports can have substantial implications, the F1-score serves as a cornerstone of our evaluation.

   
 
   
\end{itemize}

% \begin{itemize}
%     \item \textbf{Performance metrics: }
   

%     \item \textbf{Effort metrics: }
%     In our research, "readability" and "identifiability" go beyond being mere objectives; they serve as effort metrics that form an integral part of our analysis. These two aspects are not isolated from each other; instead, they work in synergy to enhance the quality of our bug report identification process.

%     Throughout RQ1 to RQ4, the metrics for readability and identifiability are assessed using the formulas contained within Section~\ref{sec:method}. However, in RQ5, a human-based evaluation approach is employed, where annotators provide individual scores for each bug report, specifically focusing on their readability and identifiability. The scores, ranging from 1 to 5, reflect the annotators' perceptions, with higher scores indicating a higher level of perceived readability or identifiability. This multifaceted approach ensures a comprehensive analysis of these essential metrics in our experiments.
        
% \end{itemize}


\subsubsection{Effort (Quantitative)}

It is also important to measure the efforts required to label the reports as part of \approach. Quantitatively, we do so by directly using the metrics for readability and identifiability of the queried report during \textit{Timestep} $n$, as discussed in Section~\ref{sec:sampling}. 

\subsubsection{Effort (Qualitative)}

Although the metrics for readability and identifiability used within the sampling of \approach~can indicate the difficulty of the reports that required labeling, they do not reflect how humans think about the effort in the real scenario. To reflect that, we design Likert scale questions that ask one to individually rate the readability and identifiability that are queried to the developers. For each attribute, the question covers five qualitative scores where a higher score indicates a more perceived readability or identifiability. We will further discuss this in Section~\ref{sec:rq5}.

In addition to the above, we also measure the time taken and monetary cost for the developers to label the queried reports recommended by \approach.

\subsection{Statistical Validation}
\label{sec:sta}

To ensure the comparative results are meaningful, we leverage the following statistical methods.

\subsubsection{Scott-Knott Test}
For comparing multiple approaches, we apply the Scott-Knott test~\cite{DBLP:journals/tse/MittasA13,scott1974cluster}---a hierarchical clustering algorithm---to determine if there are statistically meaningful differences among them. In the context of our study, we employ the Scott-Knott test to ascertain if there are significant differences in the values of metrics and hence generate a ranking across different approaches. Formally, Scott-Knott test aims to find the best split by maximizing the difference $\Delta$ in the expected mean before and after each split:
\begin{equation}
    \Delta = \frac{|l_1|}{|l|}(\overline{l_1} - \overline{l})^2 + \frac{|l_2|}{|l|}(\overline{l_2} - \overline{l})^2
\end{equation}
whereby $|l_1|$ and $|l_2|$ are the sizes of two sub-lists ($l_1$ and $l_2$) from list $l$ with a size $|l|$. $\overline{l_1}$, $\overline{l_2}$, and $\overline{l}$ denote their mean.


Recursively, in each iteration, two approaches are placed into different ranks if the results of their 10 repeated runs do not differ much according to the $\hat{A}_{12}$ effect size~\cite{Vargha2000ACA}; otherwise, they are said statistically similar. By leveraging the Scott-Knott test, we ensure that any differences observed in our results are statistically meaningful with indications of the better and worse while not requiring post-hoc correction. 

%This adds a layer of confidence to our findings, ensuring that they are not influenced by outliers or random fluctuations.

\subsubsection{Wilcoxon Sign-rank Test} We apply the Wilcoxon Sign-rank test~\cite{Wilcoxon1945IndividualCB} with $a=0.05$~\cite{DBLP:conf/icse/ArcuriB11} to investigate the statistical significance of the pairwise comparisons over all 10 runs where applicable, as it is a non-parametric statistical test that makes little assumption about the data distribution and has been recommended in software engineering research~\cite{DBLP:conf/icse/ArcuriB11}. It also assumes paired comparison between data points that fit our needs, since an individual run is completed with an independent seed.


%\subsubsection{Effect Size}

%To ensure that a $p<0.05$ is not caused by a trivial amount of the samples, we apply $\hat{A}_{12}$ effect size~\cite{Vargha2000ACA} to measure the effect size. In this work, $\hat{A}_{12}>0.5$ denotes one approach wins wherein it has a better metric value for more than 50\% of the runs. $\hat{A}_{12} \geq 0.6$ or $\hat{A}_{12} \leq 0.4$ indicate a non-trivial effect size. 

%Since there are 100 runs (instead of the commonly used 30), we use a stricter interpretation by which $0.6 \leq \hat{A}_{12} < 0.7$ (0.3 < $\hat{A}_{12} \leq 0.4$), $0.7 \leq \hat{A}_{12} < 0.8$ (0.2 < $\hat{A}_{12} \leq 0.3$), and $\hat{A}_{12} \geq 0.8$ ($\hat{A}_{12} \leq 0.2$) indicate small, medium, and large effect, respectively.

% While it's crucial to determine if differences are statistically significant, it's equally important to gauge the magnitude of these differences. This is where the A12 effect size comes into play.

% The A12 effect size provides a measure of the magnitude of difference between two sets of results~\cite{vargha2000critique}. In our study, it helps quantify how much better one method is compared to another. For each pair of configurations or methods, we calculate the A12 effect size based on their performance metrics. A value close to 1 indicates that one method consistently outperforms the other, while a value close to 0.5 suggests that the two methods perform similarly.

% The A12 effect size complements the findings from the Scott-Knott test. While the latter determines if differences are significant, the A12 effect size quantifies the magnitude of these differences. Together, they provide a comprehensive view of our method's performance relative to other approaches.

% The combination of the Scott-Knott test and the A12 effect size ensures that our findings are both statistically significant and practically meaningful. These methods provide a rigorous framework for evaluating our results, ensuring that our conclusions are well-founded and reliable.



% \subsection{Data Processing}

% We preprocessed all collected reports via the steps below: 



%By adhering to this rigorous experimental rig, we aim to provide results that are both reliable and replicable, laying a solid foundation for our findings and conclusions.

% \subsection{Ground Truth}
% The concept of "ground truth" plays a important role in our study, serving as the benchmark against which our method's performance is evaluated. However, it's essential to note that our interpretation of "ground truth" varies across different research questions (RQs):

% For RQ1-RQ4, the "ground truth" is derived from the existing labels in the dataset, categorizing reports as either "bug report" or "non-bug report." This approach simulates the manual annotation process typically encountered in active learning. By leveraging these pre-existing labels, we aim to understand how well our method can replicate or even enhance the manual annotation process, making it more efficient and accurate.

% For RQ5, our perspective on "ground truth" shifts. Here, the "ground truth" is not based on pre-existing labels but is instead determined by human annotators. We organized dedicated sessions where experts in software development carefully labeled reports as "bug-fixing" or "non-bug-fixing." This approach provides a more authentic and real-world perspective, allowing us to gauge the true efficacy of our method when faced with raw, unlabeled data.

% By adopting these dual interpretations of "ground truth," our study offers a comprehensive assessment of our proposed method. It not only evaluates the method's ability to work with pre-labeled data but also its performance when confronted with real-world, unlabeled reports.


==> sec/related.tex <==
\section{Related Surveys}
\label{sec:related}
One of the earliest surveys related to bug report analysis in general was conducted by \citeauthor{DBLP:journals/tr/StrateL13}~\cite{DBLP:journals/tr/StrateL13} in 2011, covering 104 studies. Although the paper's title suggests a focus on software defect reporting, its review actually seeks to explore the connections among various domains related to bugs/defects, such as bug report analysis, bug detection, and bug repair, instead of solely concentrating on bug report analysis. Similarly, in 2015, \citeauthor{Zhang2015}~\cite{Zhang2015} have reviewed work specifically on analyzing bug report, including papers published before or in 2014. Their focus has been on providing a comprehensive overview of the different problems in bug report analysis. Interestingly, the above reviews have not followed the systematic protocol as what we use in this work.

There also exist surveys on specific problem in bug report analysis, e.g., bug prioritization \cite{DBLP:journals/air/UddinGDNS17}, bug report summarization \cite{DBLP:conf/icetc/TararAB19} and severity prediction \cite{DBLP:journals/infsof/GomesTC19}, as opposed to the entire bug report analysis domain.

A more recent survey on bug report analysis was conducted by \citeauthor{8466000}~\cite{8466000}. Their purpose is to understand whether the problems in bug report analysis are important from the perspective of industrial practitioners. As part of the process, they carried out a systematic review on 121 studies with the sole aim to identify all the problems that are being investigated. The result of that review forms the basis to design a questionnaire for the developers to rank their importance.


In contrast, our work differs from the above in the following:

\begin{itemize}
    \item Unlike others, we seek to systematically understand what, how, why and where machine learning algorithms are used and assessed for all problems in bug report analysis. Thus our work is in fact complementary to the work by \citeauthor{8466000}~\cite{8466000}, as well as to those problem specific surveys~\cite{DBLP:journals/air/UddinGDNS17,DBLP:conf/icetc/TararAB19,DBLP:journals/infsof/GomesTC19}.
    \item Albeit machine learning based methods have been briefly discussed by \citeauthor{DBLP:journals/tr/StrateL13}~\cite{DBLP:journals/tr/StrateL13} and \citeauthor{Zhang2015}~\cite{Zhang2015}, our review captures the latest trends and provides much more comprehensive overview on this specific direction, particularly on the algorithms used, feature representation and evaluation procedure, \emph{etc}., which have been ignored in prior surveys.
    % \item We identify and justify the concerning practices on bug report analysis with machine learning, which have not been systematically discussed before, supported with evidences. 
\end{itemize}

%Zhang et al. \cite{Zhang2015} presents a survey on the work on bug-report analysis published before or in 2014. They reviewed the work by providing some background for bug reports and giving a small empirical study to motivate the necessity for work on bug-report analysis. Then they summarized the existing work on bug-report analysis and points out some possible problems in working with bug-report analysis.

%Zou et al. \cite{8466000} conducted a questionnaire among 327 practitioners to rate the importance of such techniques and provide the rationale. They also conducted follow-up interviews with 25 interviewees to gained a better understanding of the perceived usefulness (or its lack) of different categories of automated bug report management techniques. Finally, they summarized some potential research directions to help developers manage bug reports based on the finding in the survey.

%Strate et al. \cite{DBLP:journals/tr/StrateL13}  evaluated 104 academic papers on defect reporting identify the most important advancements in improving software reliability though the efficient identification and tracking of software defects. They categorized the research area into several classes and summarize the most important work being. Finally, they provided conclusions on the current state of the literature, suggest tools and lessons learned from the done in each area, and comment on open research problems.

%The three listed related surveys differ from ours in the following aspects: 1) they focus on bug report analysis using any methods whilst explicitly target ML based bug report analysis. This allows us to elaborate more detailed data and findings that have not been discussed in their work, e.g., the features and validation methods. 2) We disclose and confirm the bad smells, supported with data and justification, which prove that these are indeed the problematic practices in the field and should receive more attention as part of the future work.

==> sec/smell.tex <==
\section{Findings in the Practice from Current Work}

\label{sec:smell}

\subsection{Finding 1}

From Section~\ref{sec:RQ1-1}, we observe that the bias towards the CNNs, LSTMs, $k$NN, NB and SVM for bug report analysis is considerably large, and they have been used for decades in other fields, which suffer some known issues~\cite{seeger2000relationships,cunningham2007k,rish2001empirical}. This could be a potential concerning practice, for which we seek to verify \textit{\textbf{whether the most widely used machine learning algorithm(s) has been selected justifiably?}}

\subsubsection{Further investigation}

We revisited the studies and specifically looked for the reasons behind the choice of CNNs, LSTMs, $k$NN, NB and SVM. Inspired by the guidance introduced by \citeauthor{zhang2003machine}~\cite{zhang2003machine}, we say the choice in a study is well-justified if either of the following criteria is satisfied:

\begin{itemize}
    \item The strengths and weaknesses of the algorithms have been discussed with respect to the problem.
    \item The algorithm is selected and supported by quantitative comparison with at least one other alternative.
\end{itemize}

The results are rather positive: we found 11 well-justified cases in the studies for CNN, 5 for LSTM, 20 for $k$NN, 24 for NB and 20 for SVM. This suggests that the community is aware of their pros and cons, whilst they work surprisingly well on most problems in bug report analysis. Our finding therefore invalidates:

\begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt] 
\textbf{Practice 1:} The fact that there is a bias towards selecting $k$NN, NB and SVM is not a concerning practice, as at most of the time they are selected with good justification.
\end{tcolorbox}

\subsection{Finding 2}

In Section~\ref{sec:RQ1-2}, Word2Vec and TF-IDF, despite being popular, face significant drawbacks: Word2Vec struggles with capturing the meanings of words in different contexts (polysemy), leading to inadequate representation for words with multiple meanings. TF-IDF has a limitation on the bag-of-word representation of the text, which ignores the order and semantics of words~\cite{jonsson2016automatic}. This could be a potentially concerning practice, as fundamentally a bug report is a script of natural language. It is thus reasonable to ask \textit{\textbf{whether the choice of Word2Vec and TF-IDF has been justified.}}

\subsubsection{Further investigation}

To verify this concerning practice, we revisited the studies that use TF-IDF and looked for whether its selection has been well-justified. Inspired by the work of \citeauthor{zhang2003machine}~\cite{zhang2003machine}, we say a well-justified choice was made if it meets either of the following criteria:

\begin{itemize}
    \item Its strengths and weaknesses have been discussed with respect to the problem.
    \item It has been quantitatively compared with at least one other alternative.
    \item Unlike the machine learning algorithms that are usually alternative, methods for feature representation are often complementary. We therefore say the selection is well-justified if it is used in conjunction with other methods, e.g., Word2Vec~\cite{lilleberg2015support,ge2017improving}.
\end{itemize}


Out of the 43 studies that utilize Word2Vec and the 39 studies that utilize TF-IDF, we identified 21 and 18 studies, respectively, that do not meet any of the criteria mentioned above. At first glance, this seems to be a large proportion as it constitutes nearly 50\% of the cases. However, if this is interpreted in Figure~\ref{fig:RQ1-2}, we see that the Word2Vec and TF-IDF remain the most popular two after ruling out the 13 cases, even presuming that all others have been fully justified. This means even though certain usage of Word2Vec and TF-IDF appears to be unjustifiable, their existence does not affect the fact that Word2Vec and TF-IDF are the most predominantly used methods. The reasons include it is highly desirable in certain aspects (e,g., computational requirement as stated in some studies) or it works well in complement to other methods for bug report analysis, despite having clear limitations. Our finding thus suggests:

\begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt] 
\textbf{Practice 2:} The fact that there is a large bias towards using Word2Vec and TF-IDF is not a concerning practice, because a sufficiently high number of well-justified studies has secured it as the most popular feature representation method.
\end{tcolorbox}

\subsection{Finding 3}

From Section~\ref{sec:RQ2}, we have learned that in general, only the Eclipse and Mozilla exhibit much higher popularity than the others when evaluating a machine learning solution. We also observe that the most commonly evaluated number of projects are three and four, in which Eclipse and Mozilla are often used. When a small set of projects is evaluated (e.g., three or four), this could become a potentially concerning practice, as the large bias on these two may give a misleading impression that they sufficiently represent a good spectrum of the possible projects in the evaluation, implying that other projects can be simply omitted which may be harmful to the external validity~\cite{DBLP:conf/icse/SiegmundSA15}. We therefore ask \textit{\textbf{Whether such a large bias of selected projects in evaluation is beneficial to the coverage such that the results can be well-generalized?}}  

%\begin{table}[t!]
%	\centering
%	\caption{\# studies with reasons of using Eclipse and Mozilla.}
%	\label{tab:project-reason}%
	%\begin{threeparttable}
 %   \footnotesize
%	\begin{tabular}{ccc}\toprule
%	\textbf{Reasons}&\textbf{Eclipse}&\textbf{Mozilla}\\\midrule
%	Required by problem&8&7\\
%	Open sourced&17&13\\
%	Unknown&17&14\\
 %   \bottomrule
%	\end{tabular}
	
%\end{table}%


\begin{table}
\centering
  \caption{Coverage score (median) of studies with/without Eclipse and/or Mozilla. We use Mann-Whitney U ($\alpha=.05$)~\cite{mann1947test} for statistical test and Pearson $r$~\cite{cohen2013statistical} for effect size.}
  \label{tb:coverage}
  \footnotesize
  \begin{tabular}{lllll}
    \toprule
    \textbf{Dimension}&\textbf{with}&\textbf{without}&\textbf{$p$ value}&\textbf{$r$}\\
    \midrule
    \rowcolor{red!50}Programming language&.689&.528&.003&.28\\
    \rowcolor{green!50}Lines-of-code&.292&.594&.001&.34\\
    \rowcolor{green!50}Contributors in 12 months&.528&.580&.034&.19\\
    Code added in 12 months&.377&.458&.161&.10\\
    Code removed in 12 months&.434&.434&.211&.08\\
    \rowcolor{green!50}Comments in 12 months&.453&.514&.030&.19\\
    \rowcolor{green!50}Projects activity&.594&.792&.022&.21\\
    All dimensions&.047&.057&.201&.08\\
  \bottomrule
\end{tabular}
	\begin{tablenotes}
    \footnotesize
    \item \textcolor{red}{red} and \textcolor{green}{green} indicate the studies with Eclipse/Mozilla have higher and lower coverage than those without, respectively, under $p<.05$ and non-trivial effect size ($r>.10$) (Not edited yet).
\end{tablenotes}
\end{table}

\subsubsection{Further investigation}

To verify this concerning practice, we revisited the studies to understand why Eclipse and Mozilla were selected in the first place by looking into the paper and their dataset. The purpose is to confirm whether the reasons behind the popularity of Eclipse and Mozilla are simply because they have certain unique characteristics that are required for the problems investigated (e.g., only they have the bug types). As a result, we found only a limited number of studies made use of Eclipse (8 studies) and Mozilla (7 studies) because they fit some special needs; others (17 and 13 studies, respectively) mainly state the reasons as they are being open sourced, which is a very common property of many projects. There is also a considerable number of studies that do not give clear reasons at all (17 and 14 studies, respectively). If we rule out the cases of using Eclipse and Mozilla that are because they are open sourced or for unknown reasons, then the popularity ranking in Figure~\ref{fig:RQ2} would change dramatically\footnote{We have also found that majority of the other top 10 projects were chosen to fit specific needs, but details are omitted due to space constraint.}. This suggests that the requirement for some special needs is not the key reason behind their predominant usage.


Next, we seek to understand whether the bias towards these two projects is due to the fact that they are good representatives of the others. To this end, we make use of the coverage metric proposed by \citeauthor{DBLP:conf/sigsoft/NagappanZB13}~\cite{DBLP:conf/sigsoft/NagappanZB13} to calculate the score for each individual study. In a nutshell, this metric calculates the percentage of projects in a population that are similar to the given sample. There are two basic concepts:

\begin{itemize}
    \item \textbf{Universe:} The set of total projects for which one seeks to analyze the coverage. 
    \item \textbf{Dimension:} A feature that characterizes the projects, such as the \emph{programming language}, \emph{lines-of-code}, \emph{etc}.
\end{itemize}


\citeauthor{DBLP:conf/sigsoft/NagappanZB13}~\cite{DBLP:conf/sigsoft/NagappanZB13} define that two projects are similar on a given dimension, denoted as $d_1$ and $d_2$, if $d_1=d_2$ (for categorical dimensions, such as the \emph{programming language}) or $|log_{10}d_1 - log_{10}d_2| \leq 0.5$ (for numeric dimensions, such as the \emph{lines-of-code}). Drawing on such, two projects are said to be similar (thus they are ``covered" and ``represented" by each other) when all of their dimensions are similar. Therefore, the coverage score of a study is computed as $P_{cover} \over {P_{universe}}$, whereby $P_{universe}$ is the number of projects in the defined universe, and $P_{cover}$ is the number of projects used in a study plus the number of their similar projects from the universe.

%\begin{figure}[t!]
 % \centering
%\includestandalone[width=0.7\columnwidth]{tikz/coverage}
 %  \caption{Coverage scores for all primary studies}
 %\label{fig:coverage}
%\end{figure}

% the coverage scores on all dimensions are fairly low

Since our review covers the studies for bug report analysis with machine learning, in this work, we define the universe as all the projects evaluated in the primary studies. We use the same set of dimensions as used by \citeauthor{DBLP:conf/sigsoft/NagappanZB13}~\cite{DBLP:conf/sigsoft/NagappanZB13}. The coverage scores of studies with Eclipse or Mozilla and those that without have been shown in Figure~\ref{tb:coverage}. As can be seen, the studies consider Eclipse and/or Mozilla achieve lower coverage than those without over all but one dimension, which is programming language. Five of these comparisons are statistically significant with non-trivial effect sizes. The results imply that the large bias towards using Eclipse and Mozilla can be in fact more harmful than beneficial, as they do not provide better coverage over the spectrum of software for bug report analysis as opposed to what was believed to be.

We would like to stress that we are not asking one to discard Eclipse and Mozilla nor question their importance, as they can still be good benchmarks. What our finding suggests is that the large bias towards these two projects, together with the fact that three projects are often considered in total, implies most studies tend to wrongly believe that they are good representatives of the others and thus ignoring the other projects which could have been evaluated together. This is especially true as we have shown that the reasons behind their choices are mostly unclear. The finding therefore indicates:

\begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt] 
\textbf{Practice 3:} When using machine learning to analyze bug reports, the fact that the evaluated projects are biased towards Eclipse and/or Mozilla is a concerning practice, as it neither provides sufficiently justifiable reasons nor is representative enough, but tends to encourage the ignorance of other projects which harms the coverage.
\end{tcolorbox}


%the coverage scores on all dimensions are fairly low. Indeed, as \cite{DBLP:conf/sigsoft/NagappanZB13} pointed out, a low overall coverage score may not be bad, as it may simply be a result of low coverage on certain dimensions, while still having high coverage on the others. 

%However, we note that such a low overall coverage is in fact the result of low coverage (the median in particular) across all the dimensions considered. This raises a concern on the coverage of projects used for bug report analysis with machine learning may be indeed weak, as to improve generalizability, efforts are required on all the dimensions considered. It is also worth noting that our universe is small but specific, and therefore the low coverage scores can imply even greater problems on the generalizability of evaluation. Note that the low coverage also implies no standard benchmark available, or no such a benchmark indeed exist but have not been well-recognized. This is because if such a benchmark exists and used widely, then the coverage score would expected to be high, as the projects in the benchmark would serve as the representatives of the others. Our finding thereby suggests:





% compared with the results report in \cite{DBLP:conf/icse/MenezesP18} for the score on two years' ICSE/FSE papers.

\subsection{Finding 4}

From Section~\ref{sec:RQ3}, we have seen that certain problems are much more popular to be addressed by using machine learning. However, since software engineering research is mainly driven by practical problems, such a large bias becomes a potential concerning practice, as it implies that not all of the problems are equally important. It is thereby conservative to ask: \textit{\textbf{whether there is a discrepancy between the popularity of problems tackled by machine learning and their practically relative importance?}}


\subsubsection{Further investigation}

To answer this question and verify the concerning practice, we first revisited the primary studies to look for reasons behind the chosen problem that is tackled by machine learning. Unsurprisingly, all the studies involve at least one sentence that declares that the problem they investigated is a very important issue faced by developers.

Next, we turn to a recent comprehensive survey about the importance of various bug report analysis problems in the industry, conducted by \citeauthor{8466000}~\cite{8466000} in 2018. In the survey, a questionnaire was sent to 327 software practitioners who have experience in using bug reports to fix bugs. As part of the results, \citeauthor{8466000}~\cite{8466000} have concluded a rank on the importance of 10 bug report analysis problems (and their solutions), as shown in Table~\ref{tab:top_issue}.

Surprisingly, comparing Table~\ref{tab:2} and~\ref{tab:top_issue}, we found a rather clear discrepancy between the popularity of problems from primary studies and their practically relative importance: for the four top ranked problems by the software practitioners as the most important problems, bug localization is merely among the second widely researched issues whilst duplicate detection has have received significantly less attention than the others in the academia. Further, the two other problems, i.e., bug report completion/refinement and bug-commit linking, have rarely been researched by using machine learning in the past five years. The most popular problems from Table~\ref{tab:2} (except bug localization) are ranked much less important than duplicate detection in the practice as can be seen from Table~\ref{tab:top_issue}. The result is surprising, and one possible explanation for this could be that problems like bug categorization are much easier to be modeled as a general classification problem, in which machine learning has a long successful story. 



%In contrast, problems like bug localization is more code and engineering related, which makes the specialization of machine learning more difficult. 


We would like to emphasize that we do not intend to question the usefulness of existing work on bug report analysis with machine learning, because problems like bug categorization remain useful as appreciated by the practitioners~\cite{8466000}. However, albeit machine learning for bug report analysis has been studied for more than a decade (as reported by \citeauthor{Zhang2015}~\cite{Zhang2015}), our result implies that until now most of the studies tend to live in the ``comfort zone" to select the problems for machine learning, with little respect to their relative importance in practice. The finding therefore suggests:

\begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt] 
\textbf{Practice 4:} The popularity of currently studied problems addressed by machine learning implies a concerning practice to the field in the long term, as it largely diverts from their relative importance from the industry's perspective.
\end{tcolorbox}

%our review results disclose an concern: in the past 5 years, the most popular research problems on bug report analysis tackled by machine learning may not be consistent with the most important problems that are more urgently demanding a solution in the industry. Therefore, with the increasing exploration of machine learning algorithms, we urge the community to look more on problems of bug report analysis that are the most practically demanding.

\begin{table}[t!]
	\centering
	\caption{Importance ranking of 10 problems on bug report analysis from the industry~\cite{8466000}.}
	%\begin{threeparttable}
    \footnotesize
	\begin{tabular}{cp{7cm}}\toprule
	\textbf{Rank}&\textbf{Problem}\\\midrule
    1& Bug localization, Duplicate detection, Bug report completion/refinement, Bug-Commit linking\\
    2&Bug assignment, Bug categorization\\
    3&Bug report summarization/visualization, Bug severity/priority prediction\\
    4&Bug fixing time prediction, Re-opened bug prediction\\
    \bottomrule
	\end{tabular}
	%\end{threeparttable}
	\label{tab:top_issue}%
\end{table}%

\subsection{Finding 5}

From Section~\ref{sec:RQ4}, the results of RQ4 suggest a clear bias towards the general bug types, but a more important fact is that we found no explicit statement about performance bugs in all the studies. In this work, we define performance bugs as ``the programming errors that cause significant performance degradation”~\cite{DBLP:conf/msr/NistorJT13}. While the other minority of bug types may receive much less attention due to their rare existence, many prior studies~\cite{DBLP:conf/msr/NistorJT13,DBLP:conf/msr/ZamanAH12,DBLP:conf/msr/ZamanAH11,DBLP:conf/sosp/YinMZZBP11} have shown that performance bugs are prevalent over different software systems (e.g., Eclipse and Mozilla) and deemed as more important than the others. This could indicate a concerning practice. We thereby ask \textit{\textbf{whether the bug reports for performance bugs have indeed been ignored?}}

\subsubsection{Further investigation}



%\begin{itemize}
 %   \item Create more serious impacts to the stakeholders. \citeauthor{DBLP:conf/msr/ZamanAH12}~\cite{DBLP:conf/msr/ZamanAH12} report that, in Firefox, 8\% of the users who suffer performance bugs became frustrated enough to (threaten to) switch to another product, compared to only 1\% for non-performance bugs. 
  %  \item Take at least 32\% more time on average to fix~\cite{DBLP:conf/msr/ZamanAH11}.
   % \item Result in greater consequences. It has been reported that performance bugs accounted for 27\% of all the customer-support cases in a major storage company in the U.S., and were the most significant contributor (31\%) among all the high-severity cases~\cite{DBLP:conf/sosp/YinMZZBP11}.
%\end{itemize}

To investigate this, we revisited the 188 studies that have no declaration of the bug types. In this way, we aim to understand whether their approaches can be equally applied to performance bugs. This was conducted by looking at the assumption they made on the bug report, and the dataset they used in the evaluation. Overall, we found no evidence to suggest that the studies that tackle general bugs cannot be applied to analyze the reports on performance bugs. The only conclusion we draw for certain is that the performance bugs have not been treated differently from the other bugs. Yet, as studied by \citeauthor{DBLP:conf/msr/NistorJT13}~\cite{DBLP:conf/msr/NistorJT13} and \citeauthor{DBLP:conf/msr/ZamanAH12}~\cite{DBLP:conf/msr/ZamanAH12}, performance bugs have more readily available information in the bug report for automated analysis, which should have been explicitly catered for:

\begin{itemize}
    \item The bug reports for performance bugs with test cases, stack traces and comments are twice as many as those for non-performance bugs.
    \item Performance bugs are often found by a combination of code reasoning and behavior observations, which helps to provide a more thorough view of the root cause.
\end{itemize}

However, this is merely an opportunity for a new sub-direction rather than a concerning practice. Our finding therefore implies:


\begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt] 
\textbf{Practice 5:} The fact that the performance bug related reports have not been mentioned in machine learning based methods is not a concerning practice, as we found no evidence that the studies for general bugs cannot work on bug reports with performance bugs.
\end{tcolorbox}

%Indeed, different from most non-performance bugs, whose unexpected behaviors are clearly defined, e.g., crashes, the definition of performance bugs is vague, e.g., how slow is qualified as a performance bug? This may be a source of additional challenges. 

%This rises the opportunities for bug report analysis in machine learning. Yet, albeit the aforementioned importance and readily available foundation, our review have not found evidences that performance bugs have received sufficient attention in bug report analysis with machine learning.




%13 tfidf


\subsection{Finding 6}

From Section~\ref{sec:RQ5}, we note that precision, recall and F1-score are the predominantly used metrics in bug report analysis with machine learning. They are often evaluated with cross-validation, as shown in Figure~\ref{fig:ep}. Since the F1-score is based on precision and recall \cite{ye2018bug}, there are different ways of calculating such in the presence of repeated results (the folds). However, \citeauthor{forman2010apples}~\cite{forman2010apples} have shown that the way on how the results of different runs are aggregated can significantly impact the conclusion, which may pose a concerning practice. A question we ask is therefore \textit{\textbf{how exactly the F1-score has been calculated under repeated runs and whether it is appropriate on bug report analysis with machine learning?}}

\subsubsection{Further investigation}

\citeauthor{forman2010apples}~\cite{forman2010apples} have categoirzed three alternative ways of calculating F1-score, they are described as below:

\begin{itemize}
    \item \textbf{\texttt{Type-I}:} Here, in each fold, the F1-score ($F_i$) is recorded and the final value ($F$) is the average of all $k$ folds:
    \begin{equation}
         F={1 \over{k}} \times \sum^k_{i=1}F_i
    \end{equation}
    \item \textbf{\texttt{Type-II}:} Alternatively, one can average precision ($P_i$) and recall ($R_i$) across the folds, using their final results to compute F-measure:
    \begin{equation}
         F=2 \times {{{1 \over{k}} \sum^k_{i=1}P_i\times{1 \over{k}}\sum^k_{i=1}R_i}\over {{1 \over{k}}\sum^k_{i=1}P_i+{1 \over{k}}\sum^k_{i=1}R_i}}
    \end{equation}
    \item \textbf{\texttt{Type-III}:} Finally, instead of using some forms of average, one can use the total number of true positives ($TP_i$), false positives ($FP_i$) and false negative ($FN_i$) over the folds, then compute F1-score as if it is calculated without cross-validation:
    \begin{equation}
         F={{2 \times \sum^k_{i=1}TP_i} \over {2 \times \sum^k_{i=1}TP_i + \sum^k_{i=1}FP_i + \sum^k_{i=1}FN_i}}
    \end{equation}
\end{itemize}


According to the above categories, we revisited the primary studies and classified how they make use of F1-score and cross-validation. The results are shown in Figure~\ref{fig:fm}. After our investigation, we found that only one primary study used \texttt{Type-III}, while the other primary studies all used \texttt{Type-I} or \texttt{Type-II}. However, as~\citeauthor{forman2010apples}~\cite{forman2010apples} demonstrated, \texttt{Type-I} and \texttt{Type-II} can easily cause an unintentional and undesired bias, because they penalize methods that may occasionally predict zero positives for some test folds while smoothing out some badly performed runs by the good ones, due primarily to the nature of using mean. On the contrary, \texttt{Type-III} avoids the highly non-linear regions of the F1-score functions by considering aggregates, which provides high resilience to bias. To give a concrete example, we use the results of classifying whether a bug report indeed contains bugs, as shown in Table~\ref{tab:exp_fscore}. Here, despite the extremely good and poor precision on some runs, \texttt{Type-I} and \texttt{Type-II} would have 69\% and 73\% overall F1-score that are considerably better than 50\%, pushing it towards the good side. \texttt{Type-III}, in contrast, would only lead to 58\%, which is moderate and tends to better reflect the result. For a detailed experimental comparison, we refer the readers to~\cite{forman2010apples}. 


% \begin{figure}[t!]
%   \centering
% \includestandalone[width=0.5\columnwidth]{tikz/f-measure}
%    \caption{The ratio of different types on calculating F1-score with cross-validation.}
%  \label{fig:fm}
% \end{figure}



%This raises a concern on the construct validity of the primary studies, as misleading conclusions may be drawn based on biased results.

Another related concern is the incompatibility of results, as there is a considerable number of primary studies that calculate F1-score under cross-validation in different ways. This implies that, if researchers directly apply the F1-score reported in a study for comparison without carefully considering the calculation, then inappropriate conclusions might be drawn. Therefore, our finding suggests:

\begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt] 
\textbf{Practice 6:} The fact that \texttt{Type-I} and \texttt{Type-II} have been adopted by the majority of the studies to calculate F1-score over repeated runs poses a concerning practice, because they could lead to large bias,  and there is a lack of consistency in comparing the methods.
\end{tcolorbox}

%Therefore, we urge the practitioners of bug report analysis with machine learning to follow the suggestion by~\citeauthor{forman2010apples}~\cite{forman2010apples}, such that only \texttt{Type-III} should be used consistently when calculating F1-score under cross-validation.


\begin{table}[t!]
	\centering
	\setlength{\tabcolsep}{2mm}
	\caption{Bug categorization example to show the different calculations of F1-score over repeated runs.}
	\label{tab:exp_fscore}%
	%\begin{threeparttable}
    \footnotesize
	\begin{tabular}{ccccccccc}\toprule
	\textbf{Run/Fold}\hspace{-0.5cm}&\textbf{N}&\textbf{P}&\textbf{TP}&\textbf{FP}&\textbf{FN}&\textbf{Pr}&\textbf{Re}&\textbf{F1}\\\midrule % times 27
	1&403&108&108&0&0&100\%&100\%&100\%\\
	2&403&108&108&27&0&80\%&100\%&89\%\\
	3&403&108&108&351&0&24\%&100\%&38\%\\
	4&403&108&81&135&27&38\%&75\%&50\%\\
    \bottomrule
	\end{tabular}
	\begin{tablenotes}
    \footnotesize
    \item N, P, TP, FP, FN, Pr and Re denote the bug irrelevant reports, the bug relevant report, true positive, false positive, false negative, precision and recall, respectively.
\end{tablenotes}
	
\end{table}%

%Bug reports, being the documents that are written and submitted by human reporters, would inevitably involve strong semantic naturalness of human language. Therefore, ignoring the semantics in bug report analysis is an unwise simplification of the problem's nature. For example, in the duplicated bug reports detection problem, the summaries of two duplicated bugs reports of OpenOffice are shown as below:

%\begin{itemize}
 %   \item \textbf{Bug ID 85502:} \texttt{Alt+<letter> does not work in dialogs}
  %  \item \textbf{Bug ID 85819:} \texttt{Alt-<key> no longer works as expected}
%\end{itemize}


%As a human developer, one would know easily that they are highly likely to be duplicated reports. However, when representing feature using TF-IDF metric, the summaries of these two bug reports would have rather low similarity, since there are nearly no words that are identical. This clearly does not match with the fact. 

%Indeed, there is existing work which shows that word embedding methods, such as Word2Vec, can provide better feature representation when combined with TF-IDF ~\cite{lilleberg2015support}\cite{ge2017improving}. However, the predominated usage of sole TF-IDF still rise a concern about whether it is a reasonable choice for representing features in bug report analysis, which is often semantics related.

\subsection{Finding 7}

In Section~\ref{sec:RQ6}, Given the stochastic nature of machine learning algorithm and such a high proportion of studies without statistical test and standardized effect size, it makes sense to consider this common practice as a potential bad small and ask \textit{\textbf{are they really not required in the studies?}}


\begin{table}[t!]
	\centering
	\caption{\# repeated runs ($r$) and descriptive statistics.}
	%\begin{threeparttable}
    \footnotesize
	\begin{tabular}{cc}\toprule
	\textbf{}&\textbf{\# Studies}\\\midrule
    $0<r\leq10$&44\\
    $r>10$&26\\
    Unknown $r$&144\\
    \hline
    Reporting mean/median/best, \emph{etc}.&214\\
    Reporting full data distribution&1\\
    \bottomrule
	\end{tabular}
	%\end{threeparttable}
	\label{tab:sat-eff}%
\end{table}%


\subsubsection{Further investigation}

We revisited the studies to look for explanations on why the statistical test and effect size may not be needed. As suggested by \citeauthor{DBLP:conf/icse/ArcuriB11}~\cite{DBLP:conf/icse/ArcuriB11}, the only situation where they are not required is perhaps when (i) a sufficiently large number of repeated runs has been used and (ii) all the data points and their distributions have been reported. The results are shown in Table~\ref{tab:sat-eff}, in which we see that the majority of the studies do not clearly state how many runs are conducted; for those that do, most of them have done 10 or fewer runs. In terms of reporting, only one study has reported full distributions in addition to the descriptive statistics.

This, together with the surprisingly low usage of statistical tests and effect sizes, raises a great concern. As reported by \citeauthor{DBLP:conf/icse/ArcuriB11}~\cite{DBLP:conf/icse/ArcuriB11} and \citeauthor{DBLP:journals/infsof/KampenesDHS07}~\cite{DBLP:journals/infsof/KampenesDHS07}, their absences cannot guarantee the results were not produced by chance. This still applies when statistical test is used under a large number of runs, because it is most of the time possible to obtain statistically significant results, even if that difference is so small as to be of trivial value~\cite{DBLP:conf/icse/ArcuriB11} (standardized effect size can verify this). Our finding thus confirms:

\begin{tcolorbox}[breakable,left=5pt,right=5pt,top=5pt,bottom=5pt] 
\textbf{Practice 7:} The fact that statistical test and standardized effect size are both overwhelmingly ignored is a concerning practice, as nearly all the studies do not satisfy the conditions under which they can be confidently omitted.
\end{tcolorbox}

%In fact, the machine learning algorithms are mostly randomized and stochastic algorithm, therefore it is highly likely that the results are produced by chance, even if there are repeated runs. As discussed by \citeauthor{DBLP:conf/icse/ArcuriB11}~\cite{DBLP:conf/icse/ArcuriB11}, to evaluate randomized algorithms, researchers face with two problems: (i) how many experiments runs are required in order to obtain reliable results, and (ii) how to assess whether such results are sufficiently reliable in a rigorous way. To resolve these, the promising solution is to leverage statistical test, which measures whether the difference of two distributions are statistically significance. However, albeit that some primary studies have assessed the statistical significance, majority of them have ignored such an important procedure in the evaluation, thus leading to a concern about the reliability of the conclusion.



%The absence of effect size is even more common, but unfavorable, because, given a large enough number of runs, it is most of the time possible to obtain statistically significant results, even if that difference is so small as to be of no practical value. Therefore, standardized effect size measurements are needed, in order to assess the magnitude of the improvement in a way that is independent to the unit of metrics. In other software engineering problems, it is not uncommon to see that reporting standardized effect size is prevalent, as reported by \citeauthor{DBLP:conf/icse/ArcuriB11}~\cite{DBLP:conf/icse/ArcuriB11} and \citeauthor{DBLP:journals/infsof/KampenesDHS07}~\cite{DBLP:journals/infsof/KampenesDHS07}. As a result, the fact that only 3 primary studies have reported standardized effect size would be an immediate problem for future research in this field to address.


==> sec/why.tex <==
\section{Overcoming the Bad Practices}
\label{sec:bad}

Drawing on our findings from Section~\ref{sec:discussion}, we discuss the pragmatic resolutions to overcome the confirmed bad practices:

\begin{itemize}
    %\item \textbf{Bad smell 1:} Always provide well-justified reasons on the algorithm choice, ideally both qualitatively and quantitatively. Do not select one only because it is widely used or have been used by someone, as the popularity can lie.
    \item \textbf{Practice 2:} Considering a good number of projects to evaluate; our results show that assessing five projects could beat 67\% of the studies. Using Eclipse and Mozilla is fine, but do not choose them only because they are widely used or others believe they are good representatives of others, as the popularity can lie; justifiable reasons are required.
    \item \textbf{Practice 3:} Giving higher priority to the problems that are more important to the industry, particularly the bug duplication problem, which is deemed as one of the most important issues in the practice, but is currently under-explored with machine learning in the academia. 
    %Do not stay in the problems that are most conformable for machine learning.
    \item \textbf{Practice 6:} When F1-score is applied over repeated runs, using \texttt{Type-III} to calculate the overall result.
    \item \textbf{Practice 7:} Reporting statistical test and standardized effect size; to be on the safe side, do this for all cases. 
\end{itemize}


Indeed, some of the confirmed bad practices may not seem specific to bug report analysis with machine learning, and once identified, their resolutions may seem simple, e.g., practice 7. However, it is not easy to systematically confirm that these bad smells actually exist in this particular research field and justify that they could be crucial in the first place. This is in fact one of the key novelties of this work, which raises awareness of the community on what could be harmful but is unfortunately overlooked at the moment, thus creating potential impacts on the field.

==> tab/fig15.tex <==
% \begin{table}[t!]
% 	\centering
%         \footnotesize
% 	\setlength{\tabcolsep}{2mm}
% 	\caption{RQ1: Mean (SD) values of metrics comparing among different active learning strategies. The best value of each performance indicator is in \textcolor{red}{RED}.}
% 	\label{tab:rq1-1}%
% 	%\begin{threeparttable}
% 	\begin{tabular}{ccccccccc}\toprule
% 	\textbf{Step size}&\textbf{Methods/Metrics}\hspace{-0.5cm}&\textbf{F1-score}&\textbf{Accuracy}&\textbf{Recall}&\textbf{Precision}&\textbf{Readability}&\textbf{Identifiability}\\\midrule % times 27
  	
%    \multirow{3}{*}{300} &Random&0.858&0.851&0.848&0.869&-54.075&0.053\\
%    &Uncertainty&\textcolor{red}{0.87}&\textcolor{red}{0.862}&\textcolor{red}{0.87}&\textcolor{red}{0.87}&-37.361&0.037\\
%    &Effort&0.862&0.852&0.868&0.857&\textcolor{red}{14.894}&\textcolor{red}{0.153}\\
% \midrule
%    \multirow{3}{*}{500} &Random&0.868&0.86&0.866&0.871&-49.1&0.053\\
%    &Uncertainty&\textcolor{red}{0.874}&\textcolor{red}{0.866}&0.873&\textcolor{red}{0.875}&-41.326&0.039\\
%    &Effort&0.872&0.863&\textcolor{red}{0.878}&0.867&\textcolor{red}{-15.404}&\textcolor{red}{0.098}\\
% \midrule
%    \multirow{3}{*}{700} &Random&0.861&0.861&0.866&0.871&-53.58&0.053\\
%    &Uncertainty&\textcolor{red}{0.878}&\textcolor{red}{0.87}&0.878&\textcolor{red}{0.878}&-36.44&0.04\\
%    &Effort&0.878&0.869&\textcolor{red}{0.883}&0.873&\textcolor{red}{-11.354}&\textcolor{red}{0.093}\\
%     \bottomrule
% 	\end{tabular}	
% \end{table}%

\begin{table}[t!]
	\centering
        \footnotesize
	\setlength{\tabcolsep}{0.8mm}
	\caption{Different pseudo labeling ratio comparison for F1 scores, readability and identifiability on 10 runs. $r$ denotes the rank produced by Scott-Knott test and the statistically best results are highlighted in \setlength{\fboxsep}{1.5pt}\colorbox{teal!20}{green}.}
	\label{tab:rq1-1}%
% \resizebox{\textwidth}{!}{ % reSize the table
\begin{adjustbox}{width=\textwidth}
% \begin{tabular}{p{0.4cm}p{1.2cm}p{0.1cm}p{1.3cm}|p{0.1cm}p{1.3cm}|p{0.1cm}p{1.3cm}|p{0.1cm}p{1.3cm}|p{0.1cm}p{1.3cm}|p{0.1cm}p{1.3cm}}
\begin{tabular}{ll|llllllll|llllll}
\toprule
 \multirow{2}{*}{\textbf{Query size}} &
  \multirow{2}{*}{\textbf{Ratio}} &
  \multicolumn{2}{c}{\textbf{F1-score}} &
  \multicolumn{2}{c}{\textbf{Accuracy}} &
  \multicolumn{2}{c}{\textbf{Recall}} &
  \multicolumn{2}{c|}{\textbf{Precision}}&
  \multicolumn{2}{c}{\textbf{Readability}} &
  \multicolumn{2}{c}{\textbf{Identifiability}}\\ \cline{3-14}

 &
   &
  \textbf{$r$} &
  \textbf{Mean (SD)} &
  \textbf{$r$} &
  \textbf{Mean (SD)} &
  \textbf{$r$} &
  \textbf{Mean (SD)} &
  \textbf{$r$} &
  \textbf{Mean (SD)} &
  \textbf{$r$} &
  \textbf{Mean (SD)} &
  \textbf{$r$} &
  \textbf{Mean (SD)} \\ \midrule
%  &
%   \texttt{\approach$_{ran}$}  &3&0.858&3&0.851&3&0.848&1&\textcolor{red}{0.869}&3&-54.075&2&0.053\\
%  &
%   \texttt{\approach$_{un}$} &1&\textcolor{red}{0.87}&1&\textcolor{red}{0.862}&1&\textcolor{red}{0.87}&1&\textcolor{red}{0.87}&2&-37.361&3&0.037 \\
% \multirow{-3}{*}{300} &
%   \texttt{\approach} &2&0.864&2&0.853&2&0.873&2&0.855&1&\textcolor{red}{8.074}&1&\textcolor{red}{0.129} \\  \hline
  
%  &
%   \texttt{\approach$_{ran}$}  &3&0.868&3&0.86&3&0.866&2&0.871&3&-49.1&2&0.053\\
%  &
%   \texttt{\approach$_{un}$} &1&\textcolor{red}{0.874}&1&\textcolor{red}{0.866}&2&0.873&1&\textcolor{red}{0.875}&2&-41.326&3&0.039 \\
% \multirow{-3}{*}{500} &
%   \texttt{\approach} &2&0.872&2&0.863&1&0.878&3&0.867&1&\textcolor{red}{-15.404}&1&\textcolor{red}{0.098} \\  \hline
  
%  &
%   \texttt{\approach$_{ran}$}  &2&0.861&3&0.861&3&0.866&3&0.871&3&-53.58&2&0.053\\
%  &
%   \texttt{\approach$_{un}$} &1&\textcolor{red}{0.878}&1&\textcolor{red}{0.87}&2&0.878&1&\textcolor{red}{0.878}&2&-36.44&3&0.04 \\
% \multirow{-3}{*}{700} &
%   \texttt{\approach} &1&\textcolor{red}{0.878}&2&0.869&1&\textcolor{red}{0.883}&2&0.873&1&\textcolor{red}{-11.354}&1&\textcolor{red}{0.093}\\\bottomrule
 &
  \textbf{1}&1&0.855 ($\pm 0.018$)&1&0.847 ($\pm 0.017$)&2&0.852 ($\pm 0.031$)&1&0.859 ($\pm 0.016$)&1&1.77 ($\pm 36.207$)&1&0.167 ($\pm 0.104$)\\
 &
  \textbf{2}&1&0.856 ($\pm 0.015$)&1&0.847 ($\pm 0.015$)&2&0.856 ($\pm 0.025$)&1&0.856 ($\pm 0.015$)&1&0.447 ($\pm 38.644$)&1&0.176 ($\pm 0.119$)\\
\multirow{-3}{*}{300} &
  \textbf{3}&1&0.858 ($\pm 0.016$)&1&0.849 ($\pm 0.015$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.861 ($\pm 0.028$)&1&0.856 ($\pm 0.015$)&1&3.119 ($\pm 23.335$)&1&0.162 ($\pm 0.113$)\\  \hline
  
 &
  \textbf{1}&1&0.864 ($\pm 0.015$)&1&0.856 ($\pm 0.014$)&2&0.863 ($\pm 0.026$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.865 ($\pm 0.01$)&\cellcolor{teal!20}1&\cellcolor{teal!20}-2.511 ($\pm 18.956$)&1&0.145 ($\pm 0.106$)\\
 &
  \textbf{2}&1&0.866 ($\pm 0.013$)&1&0.857 ($\pm 0.012$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.869 ($\pm 0.021$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.864 ($\pm 0.009$)&\cellcolor{teal!20}1&\cellcolor{teal!20}-6.369 ($\pm 21.299$)&1&0.138 ($\pm 0.103$)\\
\multirow{-3}{*}{500} &
  \textbf{3}&1&0.866 ($\pm 0.012$)&1&0.856 ($\pm 0.012$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.869 ($\pm 0.019$)&2&0.862 ($\pm 0.011$)&2&-11.14 ($\pm 22.775$)&1&0.13 ($\pm 0.091$)\\  \hline
  
 &
  \textbf{1}&2&0.869 ($\pm 0.011$)&2&0.861 ($\pm 0.011$)&2&0.871 ($\pm 0.019$)&1&0.868 ($\pm 0.009$)&1&-10.555 ($\pm 18.465$)&1&0.132 ($\pm 0.1$)\\
 &
  \textbf{2}&\cellcolor{teal!20}1&\cellcolor{teal!20}0.872 ($\pm 0.011$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.863 ($\pm 0.011$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.876 ($\pm 0.019$)&1&0.868 ($\pm 0.009$)&1&-13.744 ($\pm 17.741$)&1&0.127 ($\pm 0.096$)\\
\multirow{-3}{*}{700} &
  \textbf{3}&2&0.869 ($\pm 0.011$)&2&0.86 ($\pm 0.01$)&2&0.873 ($\pm 0.018$)&1&0.866 ($\pm 0.01$)&1&-12.845 ($\pm 16.071$)&1&0.124 ($\pm 0.093$)\\  \hline


\end{tabular}
\end{adjustbox}
\end{table}%


==> tab/rq1.tex <==
\begin{table}[t!]
	\centering
        \footnotesize
	\setlength{\tabcolsep}{2mm}
	\caption{RQ1: Scott-Knott rank of metrics comparing for different active learning strategies. }
	\label{tab:rq1-1}%
	%\begin{threeparttable}
	\begin{tabular}{ccccccccc}\toprule
	\textbf{Step size}&\textbf{Methods/Metrics}\hspace{-0.5cm}&\textbf{F1-score}&\textbf{Accuracy}&\textbf{Recall}&\textbf{Precision}&\textbf{Readability}&\textbf{Identifiability}\\\midrule % times 27
  	
   \multirow{3}{*}{300} &Random&3&3&3&1&3&2\\
   &Uncertainty&1&1&1&1&2&3\\
   &Effort&2&2&2&2&1&1\\
\midrule
   \multirow{3}{*}{500} &Random&3&3&3&2&3&2\\
   &Uncertainty&1&1&2&3&2&3\\
   &Effort&2&2&1&1&1&1\\
\midrule
   \multirow{3}{*}{700} &Random&2&3&3&3&3&2\\
   &Uncertainty&1&1&2&1&2&3\\
   &Effort&1&2&1&2&1&1\\
	\end{tabular}	
\end{table}%

==> tab/rq1_avg.tex <==
% \begin{table}[t!]
% 	\centering
%         \footnotesize
% 	\setlength{\tabcolsep}{2mm}
% 	\caption{RQ1: Mean (SD) values of metrics comparing among different active learning strategies. The best value of each performance indicator is in \textcolor{red}{RED}.}
% 	\label{tab:rq1-1}%
% 	%\begin{threeparttable}
% 	\begin{tabular}{ccccccccc}\toprule
% 	\textbf{Step size}&\textbf{Methods/Metrics}\hspace{-0.5cm}&\textbf{F1-score}&\textbf{Accuracy}&\textbf{Recall}&\textbf{Precision}&\textbf{Readability}&\textbf{Identifiability}\\\midrule % times 27
  	
%    \multirow{3}{*}{300} &Random&0.858&0.851&0.848&0.869&-54.075&0.053\\
%    &Uncertainty&\textcolor{red}{0.87}&\textcolor{red}{0.862}&\textcolor{red}{0.87}&\textcolor{red}{0.87}&-37.361&0.037\\
%    &Effort&0.862&0.852&0.868&0.857&\textcolor{red}{14.894}&\textcolor{red}{0.153}\\
% \midrule
%    \multirow{3}{*}{500} &Random&0.868&0.86&0.866&0.871&-49.1&0.053\\
%    &Uncertainty&\textcolor{red}{0.874}&\textcolor{red}{0.866}&0.873&\textcolor{red}{0.875}&-41.326&0.039\\
%    &Effort&0.872&0.863&\textcolor{red}{0.878}&0.867&\textcolor{red}{-15.404}&\textcolor{red}{0.098}\\
% \midrule
%    \multirow{3}{*}{700} &Random&0.861&0.861&0.866&0.871&-53.58&0.053\\
%    &Uncertainty&\textcolor{red}{0.878}&\textcolor{red}{0.87}&0.878&\textcolor{red}{0.878}&-36.44&0.04\\
%    &Effort&0.878&0.869&\textcolor{red}{0.883}&0.873&\textcolor{red}{-11.354}&\textcolor{red}{0.093}\\
%     \bottomrule
% 	\end{tabular}	
% \end{table}%

\begin{table}[t!]
	\centering
        \footnotesize
	\setlength{\tabcolsep}{0.8mm}
	\caption{Comparing the mean and standard deviation (SD) of the metrics values for the effort-aware uncertainty sampling in \approach~and its variant counterparts that use existing samplings over all timesteps on 10 runs. $r$ denotes the rank produced by Scott-Knott test and the statistically best results are highlighted in \setlength{\fboxsep}{1.5pt}\colorbox{teal!20}{green}.}
	\label{tab:rq1-1}%
% \resizebox{\textwidth}{!}{ % reSize the table
\begin{adjustbox}{width=\textwidth}
% \begin{tabular}{p{0.4cm}p{1.2cm}p{0.1cm}p{1.3cm}|p{0.1cm}p{1.3cm}|p{0.1cm}p{1.3cm}|p{0.1cm}p{1.3cm}|p{0.1cm}p{1.3cm}|p{0.1cm}p{1.3cm}}
\begin{tabular}{ll|llllllll|llllll}
\toprule
 \multirow{2}{*}{\textbf{Query size}} &
  \multirow{2}{*}{\textbf{Approach}} &
  \multicolumn{2}{c}{\textbf{F1-score}} &
  \multicolumn{2}{c}{\textbf{Accuracy}} &
  \multicolumn{2}{c}{\textbf{Recall}} &
  \multicolumn{2}{c|}{\textbf{Precision}}&
  \multicolumn{2}{c}{\textbf{Readability}} &
  \multicolumn{2}{c}{\textbf{Identifiability}}\\ \cline{3-14}

 &
   &
  \textbf{$r$} &
  \textbf{Mean (SD)} &
  \textbf{$r$} &
  \textbf{Mean (SD)} &
  \textbf{$r$} &
  \textbf{Mean (SD)} &
  \textbf{$r$} &
  \textbf{Mean (SD)} &
  \textbf{$r$} &
  \textbf{Mean (SD)} &
  \textbf{$r$} &
  \textbf{Mean (SD)} \\ \midrule
%  &
%   \texttt{\approach$_{ran}$}  &3&0.858&3&0.851&3&0.848&1&\textcolor{red}{0.869}&3&-54.075&2&0.053\\
%  &
%   \texttt{\approach$_{un}$} &1&\textcolor{red}{0.87}&1&\textcolor{red}{0.862}&1&\textcolor{red}{0.87}&1&\textcolor{red}{0.87}&2&-37.361&3&0.037 \\
% \multirow{-3}{*}{300} &
%   \texttt{\approach} &2&0.864&2&0.853&2&0.873&2&0.855&1&\textcolor{red}{8.074}&1&\textcolor{red}{0.129} \\  \hline
  
%  &
%   \texttt{\approach$_{ran}$}  &3&0.868&3&0.86&3&0.866&2&0.871&3&-49.1&2&0.053\\
%  &
%   \texttt{\approach$_{un}$} &1&\textcolor{red}{0.874}&1&\textcolor{red}{0.866}&2&0.873&1&\textcolor{red}{0.875}&2&-41.326&3&0.039 \\
% \multirow{-3}{*}{500} &
%   \texttt{\approach} &2&0.872&2&0.863&1&0.878&3&0.867&1&\textcolor{red}{-15.404}&1&\textcolor{red}{0.098} \\  \hline
  
%  &
%   \texttt{\approach$_{ran}$}  &2&0.861&3&0.861&3&0.866&3&0.871&3&-53.58&2&0.053\\
%  &
%   \texttt{\approach$_{un}$} &1&\textcolor{red}{0.878}&1&\textcolor{red}{0.87}&2&0.878&1&\textcolor{red}{0.878}&2&-36.44&3&0.04 \\
% \multirow{-3}{*}{700} &
%   \texttt{\approach} &1&\textcolor{red}{0.878}&2&0.869&1&\textcolor{red}{0.883}&2&0.873&1&\textcolor{red}{-11.354}&1&\textcolor{red}{0.093}\\\bottomrule
 &
  \texttt{\approach$_{ran}$}  &2&0.849 ($\pm0.013$)&2&0.842 ($\pm0.011$)&2&0.837 ($\pm0.026$)&2&0.862 ($\pm0.011$)&3&-53.530 ($\pm 14.955$)&2&0.052 ($\pm0.003$)\\
 &
  \texttt{\approach$_{un}$} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.857 ($\pm 0.016$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.849 ($\pm 0.015$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.849 ($\pm 0.030$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.865 ($\pm 0.014$)&2&-36.049 ($\pm 23.043$)&3&0.041 ($\pm 0.006$)\\
\multirow{-3}{*}{300} &
  \texttt{\approach} &2&0.850 ($\pm 0.019$)&2&0.841 ($\pm 0.017$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.848 ($\pm 0.038$)&3&0.852 ($\pm 0.016$)&\cellcolor{teal!20}1&\cellcolor{teal!20}5.750 ($\pm 32.774$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.188 ($\pm 0.109$)\\  \hline
  
 &
  \texttt{\approach$_{ran}$}  &2&0.86 ($\pm 0.009$)&2&0.851 ($\pm 0.008$)&2&0.855 ($\pm 0.016$)&2&0.864 ($\pm 0.009$)&3&-53.724 ($\pm 11.302$)&2&0.053 ($\pm 0.002$)\\
 &
  \texttt{\approach$_{un}$} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.864 ($\pm 0.014$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.856 ($\pm 0.013$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.859 ($\pm 0.024$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.869 ($\pm 0.011$)&2&-35.195 ($\pm 24.862$)&3&0.040 ($\pm 0.006$)\\
\multirow{-3}{*}{500} &
  \texttt{\approach} &2&0.861 ($\pm 0.013$)&2&0.853 ($\pm 0.012$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.861 ($\pm 0.022$)&3&0.862 ($\pm 0.012$)&\cellcolor{teal!20}1&\cellcolor{teal!20}-0.119 ($\pm 20.631$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.143 ($\pm 0.087$)\\  \hline
  
 &
  \texttt{\approach$_{ran}$}  &3&0.863 ($\pm 0.008$)&3&0.855 ($\pm 0.007$)&2&0.858 ($\pm 0.016$)&2&0.868 ($\pm 0.008$)&3&-52.903 ($\pm 11.866$)&2&0.053 ($\pm 0.002$)\\
 &
  \texttt{\approach$_{un}$} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.870 ($\pm 0.009$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.861 ($\pm 0.009$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.869 ($\pm 0.016$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.871 ($\pm 0.009$)&2&-35.872 ($\pm 18.985$)&3&0.040 ($\pm 0.006$)\\
\multirow{-3}{*}{700} &
  \texttt{\approach} &2&0.867 ($\pm 0.012$)&2&0.859 ($\pm 0.012$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.869 ($\pm 0.023$)&3&0.867 ($\pm 0.011$)&\cellcolor{teal!20}1&\cellcolor{teal!20}-8.617 ($\pm 18.488$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.134 ($\pm 0.096$)\\\bottomrule


\end{tabular}
\end{adjustbox}
\end{table}%


==> tab/rq1_med.tex <==
\begin{table}[t!]
	\centering
        \footnotesize
	\setlength{\tabcolsep}{2mm}
	\caption{RQ1: Median values of metrics comparing among different active learning strategies. The best value of each performance indicator is in \textcolor{red}{RED}.}
	\label{tab:rq1-1}%
	%\begin{threeparttable}
	\begin{tabular}{ccccccccc}\toprule
	\textbf{Step size}&\textbf{Methods/Metrics}\hspace{-0.5cm}&\textbf{F1-score}&\textbf{Accuracy}&\textbf{AUC}&\textbf{Recall}&\textbf{Precision}&\textbf{Readability}&\textbf{Identifiability}\\\midrule % times 27
  	
   \multirow{3}{*}{300} &Random&0.86&0.853&0.913&0.849&0.87&-53.693&0.053\\
   &Uncertainty&0.869&0.861&0.916&0.872&0.872&-37.933&0.037\\
   &Effort&0.861&0.852&0.914&0.864&0.856&11.82&0.131\\
\midrule
   \multirow{3}{*}{500} &Random&0.868&0.859&0.912&0.868&0.87&-53.166&0.054\\
   &Uncertainty&0.874&0.865&0.915&0.873&0.874&-39.95&0.038\\
   &Effort&0.873&0.864&0.916&0.884&0.867&-5.026&0.096\\
\midrule
   \multirow{3}{*}{700} &Random&0.868&0.86&0.917&0.863&0.872&-50.818&0.054\\
   &Uncertainty&0.879&0.871&0.918&0.877&0.879&-38.777&0.04\\
   &Effort&0.879&0.87&0.923&0.885&0.871&-12.964&0.087\\
    \bottomrule
	\end{tabular}	
\end{table}%

==> tab/rq2.tex <==
\begin{table}[t!]
	\centering
        \footnotesize
	\setlength{\tabcolsep}{2mm}
	\caption{RQ2: Scott-Knott rank of metrics between using pseudo-labeling and without using pseudo-labeling. }
	\label{tab:rq1-1}%
	%\begin{threeparttable}
	\begin{tabular}{ccccccccc}\toprule
	\textbf{Step size}&\textbf{Methods/Metrics}\hspace{-0.5cm}&\textbf{F1-score}&\textbf{Accuracy}&\textbf{Recall}&\textbf{Precision}&\textbf{Readability}&\textbf{Identifiability}\\\midrule % times 27
  	
   \multirow{3}{*}{300} &With Pseudo-labeling&1&1&1&1&2&2\\
   &W/O Pseudo-labeling&2&2&2&2&1&1\\
\midrule
   \multirow{3}{*}{500} &With Pseudo-labeling&1&1&1&1&1&2\\
   &W/O Pseudo-labeling&2&2&2&2&1&1\\
\midrule
   \multirow{3}{*}{700} &With Pseudo-labeling&1&1&1&1&1&1\\
   &W/O Pseudo-labeling&2&2&2&1&1&2\\
	\end{tabular}	
\end{table}%

==> tab/rq2_avg.tex <==

% \begin{table}[t!]
% 	\centering
% 	\setlength{\tabcolsep}{2mm}
% 	\caption{RQ2: Average values of metrics comparing between using pseudo-labeling and without using pseudo-labeling. The best value of each performance indicator is in \textcolor{red}{RED}.}
% 	\label{tab:rq2-1}%
% 	%\begin{threeparttable}
%     \footnotesize
% 	\begin{tabular}{ccccccccc}\toprule
% 	\textbf{Step size}&\textbf{Methods/Metrics}\hspace{-0.5cm}&\textbf{F1-score}&\textbf{Accuracy}&\textbf{Recall}&\textbf{Precision}&\textbf{Readability}&\textbf{Identifiability}\\\midrule % times 27

%    \multirow{2}{*}{300} &With Pseudo-labeling&\textcolor{red}{0.871}&\textcolor{red}{0.862}&\textcolor{red}{0.877}&\textcolor{red}{0.866}&-2.131&0.098\\
%    &W/O Pseudo-labeling&0.862&0.852&0.868&0.857&\textcolor{red}{14.894}&\textcolor{red}{0.153}\\
% \midrule
%    \multirow{2}{*}{500} &With Pseudo-labeling&\textcolor{red}{0.878}&\textcolor{red}{0.869}&\textcolor{red}{0.883}&\textcolor{red}{0.873}&\textcolor{red}{-14.226}&0.089\\
%    &W/O Pseudo-labeling&0.872&0.863&0.878&0.867&-15.404&\textcolor{red}{0.098}\\
% \midrule
%    \multirow{2}{*}{700} &With Pseudo-labeling&\textcolor{red}{0.880}&\textcolor{red}{0.871}&\textcolor{red}{0.887}&0.873&-13.21&\textcolor{red}{0.118}\\
%    &W/O Pseudo-labeling&0.878&0.869&0.883&\textcolor{red}{0.873}&\textcolor{red}{-11.354}&0.093\\

%     \bottomrule
% 	\end{tabular}
% \end{table}%

% \begin{table}[t!]
% 	\centering
% 	\setlength{\tabcolsep}{2mm}
% 	\caption{RQ2: Average values of metrics at the final step  comparing between using pseudo-labeling and without using pseudo-labeling. The best value of each performance indicator is in green.}
% \resizebox{\textwidth}{!}{ % reSize the table
% \begin{tabular}{p{0.7cm}p{3.5cm}p{0.3cm}p{1.55cm}|p{0.3cm}p{1.55cm}|p{0.3cm}p{1.4cm}|p{0.3cm}p{1.4cm}|p{0.3cm}p{1.55cm}|p{0.3cm}p{1.4cm}}
% \toprule
%  &
%   \multirow{2}{*}{\textbf{Approach}} &
%   \multicolumn{2}{c}{\textsc{\textbf{F1-score}}} &
%   \multicolumn{2}{c}{\textsc{\textbf{Accuracy}}} &
%   \multicolumn{2}{c}{\textsc{\textbf{Recall}}} &
%   \multicolumn{2}{c}{\textsc{\textbf{Precision}}} &
%   \multicolumn{2}{c}{\textsc{\textbf{Readability}}} &
%   \multicolumn{2}{c}{\textsc{\textbf{Identifiability}}}\\ \cline{3-14}

%  &
%    &
%   \textbf{$r$} &
%   \textbf{Average} &
%   \textbf{$r$} &
%   \textbf{Average} &
%   \textbf{$r$} &
%   \textbf{Average} &
%   \textbf{$r$} &
%   \textbf{Average} &
%   \textbf{$r$} &
%   \textbf{Average} &
%   \textbf{$r$} &
%   \textbf{Average} \\ \hline
%  &
%   \texttt{w/o pseduo labeling}  &2&0.864&2&0.853&\cellcolor{teal!20}1&\cellcolor{teal!20}0.873&2&0.855&\cellcolor{teal!20}1&\cellcolor{teal!20}8.074&\cellcolor{teal!20}1&\cellcolor{teal!20}0.129\\
% \multirow{-2}{*}{300} &
%   \texttt{with pseudo-labeling} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.87&\cellcolor{teal!20}1&\cellcolor{teal!20}0.861&2&0.872&\cellcolor{teal!20}1&\cellcolor{teal!20}0.868&2&6.779&2&0.115 \\ \hline
  
%  &
%   \texttt{w/o pseduo labeling}  &2&0.872&2&0.863&2&0.878&2&0.867&2&-15.404&\cellcolor{teal!20}1&\cellcolor{teal!20}0.098\\
% \multirow{-2}{*}{500} &
%   \texttt{with pseudo-labeling} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.877&\cellcolor{teal!20}1&\cellcolor{teal!20}0.868&\cellcolor{teal!20}1&\cellcolor{teal!20}0.883&\cellcolor{teal!20}1&\cellcolor{teal!20}0.87&\cellcolor{teal!20}1&\cellcolor{teal!20}-8.392&2&0.09 \\ \hline
  
%  &
%   \texttt{w/o pseduo labeling}  &2&0.878&2&0.869&2&0.883&1&0.873&1&-11.354&1&0.093\\
% \multirow{-2}{*}{700} &
%   \texttt{with pseudo-labeling} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.880&\cellcolor{teal!20}1&\cellcolor{teal!20}0.871&\cellcolor{teal!20}1&\cellcolor{teal!20}0.887&1&0.873&1&-10.246&1&0.094\\\bottomrule

% %  &
% %   \texttt{w/o pseduo labeling}  &2&0.85&2&0.841&1&0.848&2&0.852&\cellcolor{teal!20}1&\cellcolor{teal!20}5.75&1&0.188\\
% % \multirow{-2}{*}{300} &
% %   \texttt{with pseudo-labeling} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.855&\cellcolor{teal!20}1&\cellcolor{teal!20}0.847&1&0.852&\cellcolor{teal!20}1&\cellcolor{teal!20}0.859&2&1.071&1&0.155\\ \hline
  
% %  &
% %   \texttt{w/o pseduo labeling}  &2&0.861&2&0.853&1&0.861&2&0.862&\cellcolor{teal!20}1&\cellcolor{teal!20}-0.119&1&0.143\\
% % \multirow{-2}{*}{500} &
% %   \texttt{with pseudo-labeling} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.864&\cellcolor{teal!20}1&\cellcolor{teal!20}0.856&1&0.863&\cellcolor{teal!20}1&\cellcolor{teal!20}0.865&2&-1.671&1&0.136\\ \hline
  
% %  &
% %   \texttt{w/o pseduo labeling}  &1&0.867&1&0.859&1&0.869&2&0.867&\cellcolor{teal!20}1&\cellcolor{teal!20}-8.617&1&0.134\\
% % \multirow{-2}{*}{700} &
% %   \texttt{with pseudo-labeling} &1&0.869&1&0.861&1&0.871&\cellcolor{teal!20}1&\cellcolor{teal!20}0.868&2&-9.53&1&0.122\\\bottomrule
% \end{tabular}
% }
% \end{table}%

\begin{table}[t!]
	\centering
	\setlength{\tabcolsep}{2mm}
	\caption{RQ2: Average values of metrics over ten steps comparing between using pseudo-labeling and without using pseudo-labeling. The best value of each performance indicator is in green.}
\resizebox{\textwidth}{!}{ % reSize the table
\begin{tabular}{l{0.7cm}l{3.5cm}l{0.3cm}l{1.55cm}|l{0.3cm}l{1.55cm}|l{0.3cm}l{1.4cm}|l{0.3cm}l{1.4cm}|l{0.3cm}l{1.55cm}|l{0.3cm}l{1.4cm}}
\toprule
 &
  \multirow{2}{*}{\textbf{Approach}} &
  \multicolumn{2}{c}{\textbf{F1-score}} &
  \multicolumn{2}{c}{\textbf{Accuracy}} &
  \multicolumn{2}{c}{\textbf{Recall}} &
  \multicolumn{2}{c}{\textbf{Precision}} &
  \multicolumn{2}{c}{\textbf{Readability}} &
  \multicolumn{2}{c}{\textbf{Identifiability}}\\ \cline{3-14}

 &
   &
  \textbf{$r$} &
  \textbf{Average} &
  \textbf{$r$} &
  \textbf{Average} &
  \textbf{$r$} &
  \textbf{Average} &
  \textbf{$r$} &
  \textbf{Average} &
  \textbf{$r$} &
  \textbf{Average} &
  \textbf{$r$} &
  \textbf{Average} \\ \hline
%  &
%   \texttt{w/o pseduo labeling}  &2&0.864&2&0.853&\cellcolor{teal!20}1&\cellcolor{teal!20}0.873&2&0.855&\cellcolor{teal!20}1&\cellcolor{teal!20}8.074&\cellcolor{teal!20}1&\cellcolor{teal!20}0.129\\
% \multirow{-2}{*}{300} &
%   \texttt{with pseudo-labeling} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.87&\cellcolor{teal!20}1&\cellcolor{teal!20}0.861&2&0.872&\cellcolor{teal!20}1&\cellcolor{teal!20}0.868&2&6.779&2&0.115 \\ \hline
  
%  &
%   \texttt{w/o pseduo labeling}  &2&0.872&2&0.863&2&0.878&2&0.867&2&-15.404&\cellcolor{teal!20}1&\cellcolor{teal!20}0.098\\
% \multirow{-2}{*}{500} &
%   \texttt{with pseudo-labeling} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.877&\cellcolor{teal!20}1&\cellcolor{teal!20}0.868&\cellcolor{teal!20}1&\cellcolor{teal!20}0.883&\cellcolor{teal!20}1&\cellcolor{teal!20}0.87&\cellcolor{teal!20}1&\cellcolor{teal!20}-8.392&2&0.09 \\ \hline
  
%  &
%   \texttt{w/o pseduo labeling}  &2&0.878&2&0.869&2&0.883&1&0.873&1&-11.354&1&0.093\\
% \multirow{-2}{*}{700} &
%   \texttt{with pseudo-labeling} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.880&\cellcolor{teal!20}1&\cellcolor{teal!20}0.871&\cellcolor{teal!20}1&\cellcolor{teal!20}0.887&1&0.873&1&-10.246&1&0.094\\\bottomrule

 &
  \texttt{w/o pseduo labeling}  &2&0.85&2&0.841&1&0.848&2&0.852&1&5.75&1&0.188\\
\multirow{-2}{*}{300} &
  \texttt{with pseudo-labeling} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.855&\cellcolor{teal!20}1&\cellcolor{teal!20}0.847&1&0.852&\cellcolor{teal!20}1&\cellcolor{teal!20}0.859&1&1.071&1&0.155\\ \hline
  
 &
  \texttt{w/o pseduo labeling}  &1&0.861&2&0.853&1&0.861&2&0.862&1&-0.119&1&0.143\\
\multirow{-2}{*}{500} &
  \texttt{with pseudo-labeling} &1&0.864&\cellcolor{teal!20}1&\cellcolor{teal!20}0.856&1&0.863&\cellcolor{teal!20}1&\cellcolor{teal!20}0.865&1&-1.671&1&0.136\\ \hline
  
 &
  \texttt{w/o pseduo labeling}  &1&0.867&1&0.859&1&0.869&1&0.867&1&-8.617&1&0.134\\
\multirow{-2}{*}{700} &
  \texttt{with pseudo-labeling} &1&0.869&1&0.861&1&0.871&1&0.868&1&-9.53&1&0.122\\\bottomrule
\end{tabular}
}
\end{table}%


==> tab/rq2_med.tex <==

\begin{table}[t!]
	\centering
	\setlength{\tabcolsep}{2mm}
	\caption{RQ2: Median values of metrics comparing between using pseudo-labeling and without using pseudo-labeling. The best value of each performance indicator is in \textcolor{red}{RED}.}
	\label{tab:rq2-1}%
	%\begin{threeparttable}
    \footnotesize
	\begin{tabular}{ccccccccc}\toprule
	\textbf{Step size}&\textbf{Methods/Metrics}\hspace{-0.5cm}&\textbf{F1-score}&\textbf{Accuracy}&\textbf{AUC}&\textbf{Recall}&\textbf{Precision}&\textbf{Readability}&\textbf{Identifiability}\\\midrule % times 27

   \multirow{2}{*}{300} &With Pseudo-labeling&0.872&0.862&0.918&0.877&0.865&-3.491&0.098\\
   &W/O Pseudo-labeling&0.873&0.864&0.916&0.884&0.867&-5.026&0.096\\
\midrule
   \multirow{2}{*}{500} &With Pseudo-labeling&0.878&0.87&0.916&0.883&0.872&-14.705&0.089\\
   &W/O Pseudo-labeling&0.873&0.864&0.916&0.884&0.867&-5.026&0.096\\
\midrule   
   \multirow{2}{*}{700} &With Pseudo-labeling&0.879&0.87&0.919&0.886&0.873&-12.524&0.094\\
   &W/O Pseudo-labeling&0.879&0.87&0.923&0.885&0.871&-12.964&0.087\\

    \bottomrule
	\end{tabular}
\end{table}%

==> tab/rq2_new.tex <==

% \begin{table}[t!]
% 	\centering
% 	\setlength{\tabcolsep}{2mm}
% 	\caption{RQ2: Average values of metrics comparing between using pseudo-labeling and without using pseudo-labeling. The best value of each performance indicator is in \textcolor{red}{RED}.}
% 	\label{tab:rq2-1}%
% 	%\begin{threeparttable}
%     \footnotesize
% 	\begin{tabular}{ccccccccc}\toprule
% 	\textbf{Step size}&\textbf{Methods/Metrics}\hspace{-0.5cm}&\textbf{F1-score}&\textbf{Accuracy}&\textbf{Recall}&\textbf{Precision}&\textbf{Readability}&\textbf{Identifiability}\\\midrule % times 27

%    \multirow{2}{*}{300} &With Pseudo-labeling&\textcolor{red}{0.871}&\textcolor{red}{0.862}&\textcolor{red}{0.877}&\textcolor{red}{0.866}&-2.131&0.098\\
%    &W/O Pseudo-labeling&0.862&0.852&0.868&0.857&\textcolor{red}{14.894}&\textcolor{red}{0.153}\\
% \midrule
%    \multirow{2}{*}{500} &With Pseudo-labeling&\textcolor{red}{0.878}&\textcolor{red}{0.869}&\textcolor{red}{0.883}&\textcolor{red}{0.873}&\textcolor{red}{-14.226}&0.089\\
%    &W/O Pseudo-labeling&0.872&0.863&0.878&0.867&-15.404&\textcolor{red}{0.098}\\
% \midrule
%    \multirow{2}{*}{700} &With Pseudo-labeling&\textcolor{red}{0.880}&\textcolor{red}{0.871}&\textcolor{red}{0.887}&0.873&-13.21&\textcolor{red}{0.118}\\
%    &W/O Pseudo-labeling&0.878&0.869&0.883&\textcolor{red}{0.873}&\textcolor{red}{-11.354}&0.093\\

%     \bottomrule
% 	\end{tabular}
% \end{table}%

% \begin{table}[t!]
% 	\centering
% 	\setlength{\tabcolsep}{2mm}
% 	\caption{RQ2: Average values of metrics at the final step  comparing between using pseudo-labeling and without using pseudo-labeling. The best value of each performance indicator is in green.}
% \resizebox{\textwidth}{!}{ % reSize the table
% \begin{tabular}{p{0.7cm}p{3.5cm}p{0.3cm}p{1.55cm}|p{0.3cm}p{1.55cm}|p{0.3cm}p{1.4cm}|p{0.3cm}p{1.4cm}|p{0.3cm}p{1.55cm}|p{0.3cm}p{1.4cm}}
% \toprule
%  &
%   \multirow{2}{*}{\textbf{Approach}} &
%   \multicolumn{2}{c}{\textsc{\textbf{F1-score}}} &
%   \multicolumn{2}{c}{\textsc{\textbf{Accuracy}}} &
%   \multicolumn{2}{c}{\textsc{\textbf{Recall}}} &
%   \multicolumn{2}{c}{\textsc{\textbf{Precision}}} &
%   \multicolumn{2}{c}{\textsc{\textbf{Readability}}} &
%   \multicolumn{2}{c}{\textsc{\textbf{Identifiability}}}\\ \cline{3-14}

%  &
%    &
%   \textbf{$r$} &
%   \textbf{Average} &
%   \textbf{$r$} &
%   \textbf{Average} &
%   \textbf{$r$} &
%   \textbf{Average} &
%   \textbf{$r$} &
%   \textbf{Average} &
%   \textbf{$r$} &
%   \textbf{Average} &
%   \textbf{$r$} &
%   \textbf{Average} \\ \hline
%  &
%   \texttt{w/o pseduo labeling}  &2&0.864&2&0.853&\cellcolor{teal!20}1&\cellcolor{teal!20}0.873&2&0.855&\cellcolor{teal!20}1&\cellcolor{teal!20}8.074&\cellcolor{teal!20}1&\cellcolor{teal!20}0.129\\
% \multirow{-2}{*}{300} &
%   \texttt{with pseudo-labeling} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.87&\cellcolor{teal!20}1&\cellcolor{teal!20}0.861&2&0.872&\cellcolor{teal!20}1&\cellcolor{teal!20}0.868&2&6.779&2&0.115 \\ \hline
  
%  &
%   \texttt{w/o pseduo labeling}  &2&0.872&2&0.863&2&0.878&2&0.867&2&-15.404&\cellcolor{teal!20}1&\cellcolor{teal!20}0.098\\
% \multirow{-2}{*}{500} &
%   \texttt{with pseudo-labeling} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.877&\cellcolor{teal!20}1&\cellcolor{teal!20}0.868&\cellcolor{teal!20}1&\cellcolor{teal!20}0.883&\cellcolor{teal!20}1&\cellcolor{teal!20}0.87&\cellcolor{teal!20}1&\cellcolor{teal!20}-8.392&2&0.09 \\ \hline
  
%  &
%   \texttt{w/o pseduo labeling}  &2&0.878&2&0.869&2&0.883&1&0.873&1&-11.354&1&0.093\\
% \multirow{-2}{*}{700} &
%   \texttt{with pseudo-labeling} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.880&\cellcolor{teal!20}1&\cellcolor{teal!20}0.871&\cellcolor{teal!20}1&\cellcolor{teal!20}0.887&1&0.873&1&-10.246&1&0.094\\\bottomrule

% %  &
% %   \texttt{w/o pseduo labeling}  &2&0.85&2&0.841&1&0.848&2&0.852&\cellcolor{teal!20}1&\cellcolor{teal!20}5.75&1&0.188\\
% % \multirow{-2}{*}{300} &
% %   \texttt{with pseudo-labeling} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.855&\cellcolor{teal!20}1&\cellcolor{teal!20}0.847&1&0.852&\cellcolor{teal!20}1&\cellcolor{teal!20}0.859&2&1.071&1&0.155\\ \hline
  
% %  &
% %   \texttt{w/o pseduo labeling}  &2&0.861&2&0.853&1&0.861&2&0.862&\cellcolor{teal!20}1&\cellcolor{teal!20}-0.119&1&0.143\\
% % \multirow{-2}{*}{500} &
% %   \texttt{with pseudo-labeling} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.864&\cellcolor{teal!20}1&\cellcolor{teal!20}0.856&1&0.863&\cellcolor{teal!20}1&\cellcolor{teal!20}0.865&2&-1.671&1&0.136\\ \hline
  
% %  &
% %   \texttt{w/o pseduo labeling}  &1&0.867&1&0.859&1&0.869&2&0.867&\cellcolor{teal!20}1&\cellcolor{teal!20}-8.617&1&0.134\\
% % \multirow{-2}{*}{700} &
% %   \texttt{with pseudo-labeling} &1&0.869&1&0.861&1&0.871&\cellcolor{teal!20}1&\cellcolor{teal!20}0.868&2&-9.53&1&0.122\\\bottomrule
% \end{tabular}
% }
% \end{table}%

\begin{table}[t!]
	\centering
	\setlength{\tabcolsep}{0.8mm}
	\caption{Comparing the mean and standard deviation (SD) of the metrics values for \approach~with and without pseudo-labeling over all timesteps on 10 runs. The statistically better results ($p<0.05$) are highlighted in \setlength{\fboxsep}{1.5pt}\colorbox{teal!20}{green}. $^\ast$ denotes $0.001 < p < 0.05$; $^\ddagger$ means $p \leq 0.001$.}
 	\label{tab:rq2-1}
% \resizebox{\textwidth}{!}{ % reSize the table
\begin{adjustbox}{width=\textwidth}

\begin{tabular}{ll|llll|lllll}

\toprule
\textbf{Query Size} &\textbf{Approach} &
\textbf{F1-score} &
\textbf{Accuracy} &
\textbf{Recall} &
\textbf{Precision} &
\textbf{Readability} &
\textbf{Identifiability}\\ 
%  &
%   \texttt{w/o pseduo labeling}  &2&0.864&2&0.853&\cellcolor{teal!20}1&\cellcolor{teal!20}0.873&2&0.855&\cellcolor{teal!20}1&\cellcolor{teal!20}8.074&\cellcolor{teal!20}1&\cellcolor{teal!20}0.129\\
% \multirow{-2}{*}{300} &
%   \texttt{with pseudo-labeling} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.87&\cellcolor{teal!20}1&\cellcolor{teal!20}0.861&2&0.872&\cellcolor{teal!20}1&\cellcolor{teal!20}0.868&2&6.779&2&0.115 \\ \hline
  
%  &
%   \texttt{w/o pseduo labeling}  &2&0.872&2&0.863&2&0.878&2&0.867&2&-15.404&\cellcolor{teal!20}1&\cellcolor{teal!20}0.098\\
% \multirow{-2}{*}{500} &
%   \texttt{with pseudo-labeling} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.877&\cellcolor{teal!20}1&\cellcolor{teal!20}0.868&\cellcolor{teal!20}1&\cellcolor{teal!20}0.883&\cellcolor{teal!20}1&\cellcolor{teal!20}0.87&\cellcolor{teal!20}1&\cellcolor{teal!20}-8.392&2&0.09 \\ \hline
  
%  &
%   \texttt{w/o pseduo labeling}  &2&0.878&2&0.869&2&0.883&1&0.873&1&-11.354&1&0.093\\
% \multirow{-2}{*}{700} &
%   \texttt{with pseudo-labeling} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.880&\cellcolor{teal!20}1&\cellcolor{teal!20}0.871&\cellcolor{teal!20}1&\cellcolor{teal!20}0.887&1&0.873&1&-10.246&1&0.094\\\bottomrule
\midrule
 &
  \texttt{w/o pseudo-labeling}  &0.850 ($\pm0.019$)&0.841 ($\pm0.017$)&0.848 ($\pm0.038$)&0.852 ($\pm0.016$)&\cellcolor{teal!20}5.750 ($\pm32.774$)$^\ast$&\cellcolor{teal!20}0.188 ($\pm0.109$)$^\ddagger$\\
\multirow{-2}{*}{300} &
  \texttt{w/ pseudo-labeling} &\cellcolor{teal!20}0.855 ($\pm0.018$)$^\ddagger$&\cellcolor{teal!20}0.847 ($\pm0.017$)$^\ddagger$&0.852 ($\pm0.031$)&\cellcolor{teal!20}0.859 ($\pm0.016$)$^\ddagger$&1.071 ($\pm36.207$)&0.155 ($\pm0.104$)\\ \hline
  
 &
  \texttt{w/o pseudo-labeling}  &0.861 ($\pm0.013$)&0.853 ($\pm0.012$)&0.861 ($\pm0.022$)&0.862 ($\pm0.012$)&\cellcolor{teal!20}-0.119 ($\pm20.631$)$^\ast$&0.143 ($\pm0.087$)\\
\multirow{-2}{*}{500} &
  \texttt{w/ pseudo-labeling} &\cellcolor{teal!20}0.864 ($\pm0.015$)$^\ddagger$&\cellcolor{teal!20}0.856 ($\pm0.014$)$^\ddagger$&0.863 ($\pm0.026$)&\cellcolor{teal!20}0.865 ($\pm0.010$)$^\ast$&-1.671 ($\pm18.956$)&0.136 ($\pm0.106$)\\ \hline
  
 &
  \texttt{w/o pseudo-labeling}  &0.867 ($\pm0.012$)&0.859 ($\pm0.012$)&0.869 ($\pm0.023$)&0.867 ($\pm0.011$)&-8.617 ($\pm18.488$)&0.134 ($\pm0.096$)\\
\multirow{-2}{*}{700} &
  \texttt{w/ pseudo-labeling} &\cellcolor{teal!20}0.869 ($\pm0.011$)$^\ast$&\cellcolor{teal!20}0.861 ($\pm0.011$)$^\ddagger$&0.871 ($\pm0.019$)&0.868 ($\pm0.009$)&-9.530 ($\pm18.465$)&0.122 ($\pm0.100$)\\\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}%

==> tab/rq3.tex <==
\begin{table}[t!]
	\centering
	\setlength{\tabcolsep}{2mm}
	\caption{RQ3: Scott-Knott rank of metrics between random and our method when using different pretrained language models.}

	% \label{tab:rq3-1}%
	%\begin{threeparttable}
    \footnotesize
	\begin{tabular}{cccccccccc}\toprule
	\textbf{Step size}&\textbf{Model}&\textbf{Methods}\hspace{-0.5cm}&\textbf{F1-score}&\textbf{Accuracy}&\textbf{Recall}&\textbf{Precision}&\textbf{Readability}&\textbf{Identifiability}\\\midrule % times 27

   \multirow{6}{*}{300}&\multirow{2}{*}{CodeBERT}&Random&2&2&2&2&2&2\\
   &&\approach&1&1&1&1&1&1\\\cmidrule{2-10}
   &\multirow{2}{*}{RoBERTa}&Random&2&2&2&2&2&2\\
   &&\approach&1&1&1&1&1&1\\\cmidrule{2-10}
   &\multirow{2}{*}{RTA}&Random&2&2&2&1&2&2\\
   &&\approach&1&1&1&2&1&1\\
\midrule
   \multirow{6}{*}{500}&\multirow{2}{*}{CodeBERT}&Random&2&2&2&1&2&2\\
   &&\approach&1&1&1&1&1&1\\\cmidrule{2-10}
   &\multirow{2}{*}{RoBERTa}&Random&2&2&2&2&2&2\\
   &&\approach&1&1&1&1&1&1\\\cmidrule{2-10}
   &\multirow{2}{*}{RTA}&Random&2&2&2&1&2&2\\
   &&\approach&1&1&1&1&1&1\\
\midrule
   \multirow{6}{*}{700}&\multirow{2}{*}{CodeBERT}&Random&2&2&2&1&2&2\\
   &&\approach&1&1&1&1&1&1\\\cmidrule{2-10}
   &\multirow{2}{*}{RoBERTa}&Random&2&2&2&2&2&2\\
   &&\approach&1&1&1&1&1&1\\\cmidrule{2-10}
   &\multirow{2}{*}{RTA}&Random&2&2&2&1&2&2\\
   &&\approach&1&1&&1&1&1&1\\
    \bottomrule
	\end{tabular}

\label{tab:rq3-1}
\end{table}%

==> tab/rq3_avg.tex <==
% \begin{table}[t!]
% 	\centering
% 	\setlength{\tabcolsep}{2mm}
% 	\caption{RQ3: Average values of metrics comparing between \approach$_{ran}$ and our method when using different pretrained language models. The best value of each performance indicator is in \textcolor{red}{RED}.}

% 	% \label{tab:rq3-1}%
% 	%\begin{threeparttable}
%     \footnotesize
% 	\begin{tabular}{cccccccccc}\toprule
% 	\textbf{Step size}&\textbf{Model}&\textbf{Methods}\hspace{-0.5cm}&\textbf{F1-score}&\textbf{Accuracy}&\textbf{Recall}&\textbf{Precision}&\textbf{Readability}&\textbf{Identifiability}\\\midrule % times 27

%    \multirow{6}{*}{300}&\multirow{2}{*}{CodeBERT}&\approach$_{ran}$&0.864&0.856&0.862&0.867&-49.548&0.053\\
%    &&\approach&\textcolor{red}{0.875}&\textcolor{red}{0.866}&\textcolor{red}{0.881}&\textcolor{red}{0.87}&\textcolor{red}{-13.376}&\textcolor{red}{0.113}\\\cmidrule{2-10}
%    &\multirow{2}{*}{RoBERTa}&\approach$_{ran}$&0.867&0.857&0.87&0.863&-59.287&0.052\\
%    &&\approach&\textcolor{red}{0.877}&\textcolor{red}{0.867}&\textcolor{red}{0.885}&\textcolor{red}{0.868}&\textcolor{red}{-6.543}&\textcolor{red}{0.101}\\\cmidrule{2-10}
%    &\multirow{2}{*}{RTA}&\approach$_{ran}$&0.879&0.871&0.883&\textcolor{red}{0.875}&-54.043&0.052\\
%    &&\approach&\textcolor{red}{0.886}&\textcolor{red}{0.877}&\textcolor{red}{0.897}&0.874&\textcolor{red}{-2.207}&\textcolor{red}{0.108}\\
% \midrule
%    \multirow{6}{*}{500}&\multirow{2}{*}{CodeBERT}&\approach$_{ran}$&0.869&0.861&0.867&0.872&-47.712&0.054\\
%    &&\approach&\textcolor{red}{0.88}&\textcolor{red}{0.871}&\textcolor{red}{0.887}&\textcolor{red}{0.873}&\textcolor{red}{-13.942}&\textcolor{red}{0.087}\\\cmidrule{2-10}
%    &\multirow{2}{*}{RoBERTa}&\approach$_{ran}$&0.87&0.861&0.869&0.87&-50.123&0.053\\
%    &&\approach&\textcolor{red}{0.88}&\textcolor{red}{0.871}&\textcolor{red}{0.888}&\textcolor{red}{0.872}&\textcolor{red}{-11.754}&\textcolor{red}{0.103}\\\cmidrule{2-10}
%    &\multirow{2}{*}{RTA}&\approach$_{ran}$&0.884&0.875&0.89&0.878&-56.962&0.053\\
%    &&\approach&\textcolor{red}{0.889}&\textcolor{red}{0.881}&\textcolor{red}{0.9}&\textcolor{red}{0.879}&\textcolor{red}{-11.52}&\textcolor{red}{0.129}\\
% \midrule
%    \multirow{6}{*}{700}&\multirow{2}{*}{CodeBERT}&\approach$_{ran}$&0.872&0.864&0.871&0.873&-57.184&0.052\\
%    &&\approach&\textcolor{red}{0.882}&\textcolor{red}{0.873}&\textcolor{red}{0.889}&\textcolor{red}{0.874}&\textcolor{red}{-14.614}&\textcolor{red}{0.135}\\\cmidrule{2-10}
%    &\multirow{2}{*}{RoBERTa}&\approach$_{ran}$&0.871&0.862&0.872&0.87&-47.866&0.053\\
%    &&\approach&\textcolor{red}{0.882}&\textcolor{red}{0.873}&\textcolor{red}{0.89}&\textcolor{red}{0.874}&\textcolor{red}{-15.198}&\textcolor{red}{0.117}\\\cmidrule{2-10}
%    &\multirow{2}{*}{RTA}&\approach$_{ran}$&0.884&0.876&0.889&0.879&-51.048&0.053\\
%    &&\approach&\textcolor{red}{0.889}&\textcolor{red}{0.881}&&\textcolor{red}{0.9}&0.879&\textcolor{red}{-14.105}&\textcolor{red}{0.13}\\
%     \bottomrule
% 	\end{tabular}

% \label{tab:rq3-1}
% \end{table}%

\begin{table}[t!]
	\centering
	\setlength{\tabcolsep}{2mm}
	\caption{RQ3: Average values of metrics at the final step  comparing between \approach$_{ran}$ and our method when using different pretrained language models. The best value of each performance indicator is in green.}

%all timesteps on 10 runs

% \resizebox{\textwidth}{!}{ % reSize the table
% \begin{tabular}{p{0.7cm}p{2cm}p{0.3cm}p{1.55cm}|p{0.3cm}p{1.55cm}|p{0.3cm}p{1.4cm}|p{0.3cm}p{1.4cm}|p{0.3cm}p{1.55cm}|p{0.3cm}p{1.4cm}}
% \toprule
% &
%   \multirow{2}{*}{\textbf{Model}} &
%   \multirow{2}{*}{\textbf{Approach}} &
%   \multicolumn{2}{c}{\textsc{\textbf{F1-score}}} &
%   \multicolumn{2}{c}{\textsc{\textbf{Accuracy}}} &
%   \multicolumn{2}{c}{\textsc{\textbf{Recall}}} &
%   \multicolumn{2}{c}{\textsc{\textbf{Precision}}} &
%   \multicolumn{2}{c}{\textsc{\textbf{Readability}}} &
%   \multicolumn{2}{c}{\textsc{\textbf{Identifiability}}}\\ \cline{4-14}

%  &
%  &
%    &
%   \textbf{$r$} &
%   \textbf{Average} &
%   \textbf{$r$} &
%   \textbf{Average} &
%   \textbf{$r$} &
%   \textbf{Average} &
%   \textbf{$r$} &
%   \textbf{Average} &
%   \textbf{$r$} &
%   \textbf{Average} &
%   \textbf{$r$} &
%   \textbf{Average} & \\ \hline
%  &
%   \texttt{\approach$_{ran}$}  &1&1&1&1&1&1&1&1&1&1&1&1\\
%  &
%   \texttt{\approach} &1&1&1&1&1&1&1&1&1&1&1&1 \\
%  &
%   \texttt{\approach$_{ran}$}  &1&1&1&1&1&1&1&1&1&1&1&1\\
% \multirow{-6}{*}{300}&
%   \texttt{\approach} &1&1&1&1&1&1&1&1&1&1&1&1 \\ 
% &
%   \texttt{\approach$_{ran}$}  &1&1&1&1&1&1&1&1&1&1&1&1\\
%  &
%   \texttt{\approach} &1&1&1&1&1&1&1&1&1&1&1&1 \\\hline
  
%  &
%   \texttt{\approach$_{ran}$}  &1&1&1&1&1&1&1&1&1&1&1&1\\
%  &
%   \texttt{\approach} &1&1&1&1&1&1&1&1&1&1&1&1 \\
% \multirow{-6}{*}{500} 
%  &
%   \texttt{\approach$_{ran}$}  &1&1&1&1&1&1&1&1&1&1&1&1\\
%  &
%   \texttt{\approach} &1&1&1&1&1&1&1&1&1&1&1&1 \\ 
% &
%   \texttt{\approach$_{ran}$}  &1&1&1&1&1&1&1&1&1&1&1&1\\
%  &
%   \texttt{\approach} &1&1&1&1&1&1&1&1&1&1&1&1 \\\hline
  
%  &
%   \texttt{\approach$_{ran}$}  &1&1&1&1&1&1&1&1&1&1&1&1\\
%  &
%   \texttt{\approach} &1&1&1&1&1&1&1&1&1&1&1&1 \\
% \multirow{-6}{*}{700} 
%  &
%   \texttt{\approach$_{ran}$}  &1&1&1&1&1&1&1&1&1&1&1&1\\
%  &
%   \texttt{\approach} &1&1&1&1&1&1&1&1&1&1&1&1 \\ 
% &
%   \texttt{\approach$_{ran}$}  &1&1&1&1&1&1&1&1&1&1&1&1\\
%  &
%   \texttt{\approach} &1&1&1&1&1&1&1&1&1&1&1&1 \\\hline

 
% \bottomrule
% \end{tabular}
% }

\resizebox{\textwidth}{!}{ % reSize the table
\begin{tabular}{p{1cm}p{1.5cm}p{2cm}p{0.3cm}p{1.55cm}|p{0.3cm}p{1.55cm}|p{0.3cm}p{1.4cm}|p{0.3cm}p{1.4cm}|p{0.3cm}p{1.55cm}|p{0.3cm}p{1.4cm}}
\toprule
 \multirow{2}{*}{\textbf{Size}} &\multirow{2}{*}{\textbf{Model}} &
  \multirow{2}{*}{\textbf{Approach}} &
  \multicolumn{2}{c}{\textsc{\textbf{F1-score}}} &
  \multicolumn{2}{c}{\textsc{\textbf{Accuracy}}} &
  \multicolumn{2}{c}{\textsc{\textbf{Recall}}} &
  \multicolumn{2}{c}{\textsc{\textbf{Precision}}} &
  \multicolumn{2}{c}{\textsc{\textbf{Readability}}} &
  \multicolumn{2}{c}{\textsc{\textbf{Identifiability}}}\\ \cline{4-15}

 &
 &
   &
  \textbf{$r$} &
  \textbf{Average} &
  \textbf{$r$} &
  \textbf{Average} &
  \textbf{$r$} &
  \textbf{Average} &
  \textbf{$r$} &
  \textbf{Average} &
  \textbf{$r$} &
  \textbf{Average} &
  \textbf{$r$} &
  \textbf{Average} \\ \hline
&&
  \texttt{\approach$_{ran}$}  &2&0.864&2&0.856&2&0.862&2&0.867&2&-49.548&2&0.053\\
&\multirow{-2}{*}{CodeBERT}&
  \texttt{\approach} &1&\textcolor{red}{0.875}&1&\textcolor{red}{0.866}&1&\textcolor{red}{0.881}&1&\textcolor{red}{0.87}&1&\textcolor{red}{-13.376}&1&\textcolor{red}{0.113}\\\cline{2-15}
&&
  \texttt{\approach$_{ran}$}  &2&0.867&2&0.857&2&0.87&2&0.863&2&-59.287&2&0.052\\  
&\multirow{-2}{*}{RoBERTa}&
  \texttt{\approach}  &1&\textcolor{red}{0.877}&1&\textcolor{red}{0.867}&1&\textcolor{red}{0.885}&1&\textcolor{red}{0.868}&1&\textcolor{red}{-6.543}&1&\textcolor{red}{0.101}\\\cline{2-15}
&&
  \texttt{\approach$_{ran}$} &2&0.879&2&0.871&2&0.883&1&\textcolor{red}{0.875}&2&-54.043&2&0.052\\
\multirow{-6}{*}{300} &\multirow{-2}{*}{RTA} &
  \texttt{\approach}  &1&\textcolor{red}{0.886}&1&\textcolor{red}{0.877}&1&\textcolor{red}{0.897}&2&0.874&1&\textcolor{red}{-2.207}&1&\textcolor{red}{0.108}\\ \hline
  
&&
  \texttt{\approach$_{ran}$}  &2&0.869&2&0.861&2&0.867&1&0.872&2&-47.712&2&0.054\\
&\multirow{-2}{*}{CodeBERT}&
  \texttt{\approach} &1&\textcolor{red}{0.88}&1&\textcolor{red}{0.871}&1&\textcolor{red}{0.887}&1&0.873&1&\textcolor{red}{-13.942}&1&\textcolor{red}{0.087}\\\cline{2-15}
&&
  \texttt{\approach$_{ran}$}  &2&0.87&2&0.861&2&0.869&2&0.87&2&-50.123&2&0.053\\  
&\multirow{-2}{*}{RoBERTa}&
  \texttt{\approach}  &1&\textcolor{red}{0.88}&1&\textcolor{red}{0.871}&1&\textcolor{red}{0.888}&1&\textcolor{red}{0.872}&1&\textcolor{red}{-11.754}&1&\textcolor{red}{0.103}\\\cline{2-15}
&&
  \texttt{\approach$_{ran}$} &2&0.884&2&0.875&2&0.89&1&0.878&2&-56.962&2&0.053\\
\multirow{-6}{*}{500} &\multirow{-2}{*}{RTA} &
  \texttt{\approach}  &1&\textcolor{red}{0.889}&1&\textcolor{red}{0.881}&1&\textcolor{red}{0.9}&1&0.879&1&\textcolor{red}{-11.52}&1&\textcolor{red}{0.129}\\ \hline

&&
  \texttt{\approach$_{ran}$}  &2&0.872&2&0.864&2&0.871&1&0.873&2&-57.184&2&0.052\\
&\multirow{-2}{*}{CodeBERT}&
  \texttt{\approach} &1&\textcolor{red}{0.882}&1&\textcolor{red}{0.873}&1&\textcolor{red}{0.889}&1&0.874&1&\textcolor{red}{-14.614}&1&\textcolor{red}{0.135}\\\cline{2-15}
&&
  \texttt{\approach$_{ran}$}  &2&0.871&2&0.862&2&0.872&2&0.87&2&-47.866&2&0.053\\  
&\multirow{-2}{*}{RoBERTa}&
  \texttt{\approach}  &1&\textcolor{red}{0.882}&1&\textcolor{red}{0.873}&1&\textcolor{red}{0.89}&1&\textcolor{red}{0.874}&1&\textcolor{red}{-15.198}&1&\textcolor{red}{0.117}\\\cline{2-15}
&&
  \texttt{\approach$_{ran}$} &2&0.884&2&0.876&2&0.889&1&0.879&2&-51.048&2&0.053\\
\multirow{-6}{*}{700} &\multirow{-2}{*}{RTA} &
  \texttt{\approach}  &1&\textcolor{red}{0.889}&1&\textcolor{red}{0.881}&1&\textcolor{red}{0.9}&1&0.879&1&\textcolor{red}{-14.105}&1&\textcolor{red}{0.13}\\\bottomrule
% &&
%   \texttt{\approach$_{ran}$}  &&0.853&&0.846&&0.841&&0.866&&-51.532&&0.053\\
% &\multirow{-2}{*}{CodeBERT}&
%   \texttt{\approach} &&0.864&&0.855&&0.863&&0.865&&-5.5&&0.165\\\cline{2-15}
% &&
%   \texttt{\approach$_{ran}$}  &&0.861&&0.852&&0.86&&0.861&&-50.017&&0.053\\
% &\multirow{-2}{*}{RoBERTa}&
%   \texttt{\approach}  &&0.868&&0.858&&0.874&&0.862&&-0.473&&0.157\\\cline{2-15}
% &&
%   \texttt{\approach$_{ran}$} &&0.875&&0.866&&0.88&&0.87&&-51.317&&0.053\\
% \multirow{-6}{*}{300} &\multirow{-2}{*}{RTA} &
%   \texttt{\approach}  &&0.88&&0.871&&0.891&&0.87&&-5.331&&0.156\\ \hline
  
% &&
%   \texttt{\approach$_{ran}$}  &&0.862&&0.854&&0.855&&0.869&&-52.605&&0.053\\
% &\multirow{-2}{*}{CodeBERT}&
%   \texttt{\approach} &&0.87&&0.861&&0.872&&0.868&&-14.026&&0.135\\\cline{2-15}
% &&
%   \texttt{\approach$_{ran}$}  &&0.865&&0.856&&0.865&&0.865&&-52.01&&0.053\\
% &\multirow{-2}{*}{RoBERTa}&
%   \texttt{\approach}  &&0.873&&0.864&&0.878&&0.867&&-12.0&&0.137\\\cline{2-15}
% &&
%   \texttt{\approach$_{ran}$} &&0.88&&0.871&&0.887&&0.873&&-51.033&&0.053\\
% \multirow{-6}{*}{500} &\multirow{-2}{*}{RTA} &
%   \texttt{\approach}  &&0.884&&0.875&&0.893&&0.875&&-16.241&&0.141\\ \hline

% &&
%   \texttt{\approach$_{ran}$}  &&0.866&&0.858&&0.862&&0.871&&-54.596&&0.052\\
% &\multirow{-2}{*}{CodeBERT}&
%   \texttt{\approach} &&0.875&&0.866&&0.878&&0.871&&-13.356&&0.126\\\cline{2-15}
% &&
%   \texttt{\approach$_{ran}$}  &&0.867&&0.859&&0.867&&0.868&&-52.139&&0.053\\ 
% &\multirow{-2}{*}{RoBERTa}&
%   \texttt{\approach}  &&0.875&&0.866&&0.882&&0.869&&-16.749&&0.137\\\cline{2-15}
% &&
%   \texttt{\approach$_{ran}$} &&0.881&&0.873&&0.887&&0.875&&-51.531&&0.053\\
% \multirow{-6}{*}{700} &\multirow{-2}{*}{RTA} &
%   \texttt{\approach}  &&0.885&&0.877&&0.894&&0.877&&-16.551&&0.139\\\bottomrule

\end{tabular}
}
\label{tab:rq3-1}
\end{table}%

==> tab/rq3_med.tex <==
\begin{table}[t!]
	\centering
	\setlength{\tabcolsep}{2mm}
	\caption{RQ3: Median values of metrics comparing between random and our method when using different pretrained language models. The best value of each performance indicator is in \textcolor{red}{RED}.}

	% \label{tab:rq3-1}%
	%\begin{threeparttable}
    \footnotesize
	\begin{tabular}{cccccccccc}\toprule
	\textbf{Step size}&\textbf{Model}&\textbf{Methods}\hspace{-0.5cm}&\textbf{F1-score}&\textbf{Accuracy}&\textbf{AUC}&\textbf{Recall}&\textbf{Precision}&\textbf{Readability}&\textbf{Identifiability}\\\midrule % times 27

   \multirow{6}{*}{300}&\multirow{2}{*}{CodeBERT}&Random&0.864&0.856&0.912&0.859&0.868&-47.225&0.052\\
   &&\approach&0.877&0.867&0.921&0.881&0.871&-1.993&0.101\\\cmidrule{2-10}
   &\multirow{2}{*}{RoBERTa}&Random&0.866&0.857&0.915&0.87&0.864&-55.797&0.052\\
   &&\approach&0.878&0.869&0.911&0.885&0.868&-8.267&0.099\\\cmidrule{2-10}
   &\multirow{2}{*}{RTA}&Random&0.88&0.871&0.916&0.883&0.876&-48.425&0.052\\
   &&\approach&0.886&0.877&0.926&0.898&0.876&-6.709&0.094\\
\midrule
   \multirow{6}{*}{500}&\multirow{2}{*}{CodeBERT}&Random&0.87&0.861&0.914&0.87&0.872&-48.459&0.053\\
   &&\approach&0.881&0.872&0.914&0.889&0.874&-15.562&0.083\\\cmidrule{2-10}
   &\multirow{2}{*}{RoBERTa}&Random&0.869&0.861&0.908&0.869&0.869&-48.517&0.053\\
   &&\approach&0.879&0.871&0.906&0.886&0.874&-10.104&0.093\\\cmidrule{2-10}
   &\multirow{2}{*}{RTA}&Random&0.883&0.876&0.923&0.89&0.878&-59.071&0.053\\
   &&\approach&0.889&0.881&0.922&0.901&0.879&-12.253&0.096\\
\midrule
   \multirow{6}{*}{700}&\multirow{2}{*}{CodeBERT}&Random&0.872&0.865&0.914&0.87&0.873&-56.881&0.052\\
   &&\approach&0.882&0.873&0.91&0.89&0.874&-6.647&0.121\\\cmidrule{2-10}
   &\multirow{2}{*}{RoBERTa}&Random&0.871&0.863&0.91&0.873&0.87&-47.229&0.053\\
   &&\approach&0.881&0.873&0.912&0.889&0.875&-13.273&0.101\\\cmidrule{2-10}
   &\multirow{2}{*}{RTA}&Random&0.884&0.876&0.923&0.888&0.879&-51.703&0.053\\
   &&\approach&0.888&0.88&0.913&0.898&0.881&-17.738&0.12\\
    \bottomrule
	\end{tabular}

\label{tab:rq3-1}
\end{table}%

==> tab/rq3_new.tex <==

\begin{table}[t!]
	\centering
	\setlength{\tabcolsep}{0.8mm}
	\caption{Comparing the mean and standard deviation (SD) of the metrics values for \approach~under different neural language models against updating them directly. The format is the same as Table~\ref{tab:rq2-1}.}
\label{tab:rq3-1}
% \resizebox{\textwidth}{!}{ % reSize the table
\begin{adjustbox}{width=\textwidth}
% \begin{tabular}{p{1cm}p{1.5cm}p{2cm}p{1.55cm}|p{1.55cm}|p{1.4cm}|p{1.4cm}|p{1.4cm}|p{1.4cm}}
\begin{tabular}{lll|llll|lll}

\toprule
\textbf{Query Size} &\textbf{Model} &\textbf{Approach} &
\textbf{F1-score} &
\textbf{Accuracy} &
\textbf{Recall} &
\textbf{Precision} &
\textbf{Readability} &
\textbf{Identifiability}\\ 
% &&
% \texttt{\approach$_{ran}$} &0.853&0.846&0.841&0.866&-51.532&0.053\\
% &\multirow{-2}{*}{CodeBERT}&
% \texttt{\approach} &0.864&0.855&0.863&0.865&-5.5&0.165\\

% \cline{1-10}
\midrule
&&
  \texttt{\approach$_{ran}$}  &0.853 ($\pm0.014$)&0.846 ($\pm0.013$)&0.841 ($\pm0.025$)&0.866 ($\pm0.011$)&-51.532 ($\pm14.501$)&0.053 ($\pm0.003$)\\
&\multirow{-2}{*}{CodeBERT}&
  \texttt{\approach} &\cellcolor{teal!20}0.864 ($\pm0.016$)$^\ddagger$&\cellcolor{teal!20}0.855 ($\pm0.015$)$^\ddagger$&\cellcolor{teal!20}0.863 ($\pm0.027$)$^\ddagger$&0.865 ($\pm0.01$)&\cellcolor{teal!20}-5.500 ($\pm40.631$)$^\ddagger$&\cellcolor{teal!20}0.165 ($\pm0.118$)$^\ddagger$\\\cline{2-9}
&&
  \texttt{\approach$_{ran}$}  &0.861 ($\pm0.010$)&0.852 ($\pm0.009$)&0.86 ($\pm0.021$)&0.861 ($\pm0.010$)&-50.017 ($\pm14.424$)&0.053 ($\pm0.003$)\\
&\multirow{-2}{*}{RoBERTa}&
  \texttt{\approach}  &\cellcolor{teal!20}0.868 ($\pm0.011$)$^\ddagger$&\cellcolor{teal!20}0.858 ($\pm0.011$)$^\ddagger$&\cellcolor{teal!20}0.874 ($\pm0.017$)$^\ddagger$&0.862 ($\pm0.012$)&\cellcolor{teal!20}-0.473 ($\pm24.745$)$^\ddagger$&\cellcolor{teal!20}0.157 ($\pm0.117$)$^\ddagger$\\\cline{2-9}
&&
  \texttt{\approach$_{ran}$} &0.875 ($\pm0.007$)&0.866 ($\pm0.007$)&0.880 ($\pm0.015$)&0.870 ($\pm0.010$)&-51.317 ($\pm13.598$)&0.053 ($\pm0.003$)\\
\multirow{-6}{*}{300} &\multirow{-2}{*}{RTA} &
  \texttt{\approach}  &\cellcolor{teal!20}0.880 ($\pm0.010$)$^\ddagger$&\cellcolor{teal!20}0.871 ($\pm0.010$)$^\ddagger$&\cellcolor{teal!20}0.891 ($\pm0.017$)$^\ddagger$&0.870 ($\pm0.011$)&\cellcolor{teal!20}-5.331 ($\pm31.372$)$^\ddagger$&\cellcolor{teal!20}0.156 ($\pm0.121$)$^\ddagger$\\ \hline
  
&&
  \texttt{\approach$_{ran}$}  &0.862 ($\pm0.010$)&0.854 ($\pm0.009$)&0.855 ($\pm0.019$)&0.869 ($\pm0.008$)&-52.605 ($\pm11.605$)&0.053 ($\pm0.002$)\\
&\multirow{-2}{*}{CodeBERT}&
  \texttt{\approach} &\cellcolor{teal!20}0.870 ($\pm0.013$)$^\ddagger$&\cellcolor{teal!20}0.861 ($\pm0.012$)$^\ddagger$&\cellcolor{teal!20}0.872 ($\pm0.024$)$^\ddagger$&0.868 ($\pm0.009$)&\cellcolor{teal!20}-14.026 ($\pm24.921$)$^\ddagger$&\cellcolor{teal!20}0.135 ($\pm0.102$)$^\ddagger$\\\cline{2-9}
&&
  \texttt{\approach$_{ran}$}  &0.865 ($\pm0.008$)&0.856 ($\pm0.007$)&0.865 ($\pm0.015$)&0.865 ($\pm0.007$)&-52.010 ($\pm10.750$)&0.053 ($\pm0.002$)\\
&\multirow{-2}{*}{RoBERTa}&
  \texttt{\approach}  &\cellcolor{teal!20}0.873 ($\pm0.010$)$^\ddagger$&\cellcolor{teal!20}0.864 ($\pm0.010$)$^\ddagger$&\cellcolor{teal!20}0.878 ($\pm0.019$)$^\ddagger$&0.867 ($\pm0.008$)&\cellcolor{teal!20}-12.000 ($\pm23.367$)$^\ddagger$&\cellcolor{teal!20}0.137 ($\pm0.109$)$^\ddagger$\\\cline{2-9}
&&
  \texttt{\approach$_{ran}$} &0.880 ($\pm0.005$)&0.871 ($\pm0.005$)&0.887 ($\pm0.011$)&0.873 ($\pm0.008$)&-51.033 ($\pm10.880$)&0.053 ($\pm0.002$)\\
\multirow{-6}{*}{500} &\multirow{-2}{*}{RTA} &
  \texttt{\approach}  &\cellcolor{teal!20}0.884 ($\pm0.007$)$^\ddagger$&\cellcolor{teal!20}0.875 ($\pm0.007$)$^\ddagger$&\cellcolor{teal!20}0.893 ($\pm0.012$)$^\ddagger$&0.875 ($\pm0.008$)&\cellcolor{teal!20}-16.241 ($\pm27.093$)$^\ddagger$&\cellcolor{teal!20}0.141 ($\pm0.122$)$^\ddagger$\\ \hline

&&
  \texttt{\approach$_{ran}$}  &0.866 ($\pm0.008$)&0.858 ($\pm0.007$)&0.862 ($\pm0.015$)&0.871 ($\pm0.008$)&-54.596 ($\pm14.400$)&0.052 ($\pm0.002$)\\
&\multirow{-2}{*}{CodeBERT}&
  \texttt{\approach} &\cellcolor{teal!20}0.875 ($\pm0.010$)$^\ddagger$&\cellcolor{teal!20}0.866 ($\pm0.010$)$^\ddagger$&\cellcolor{teal!20}0.878 ($\pm0.018$)$^\ddagger$&0.871 ($\pm0.007$)&\cellcolor{teal!20}-13.356 ($\pm15.890$)$^\ddagger$&\cellcolor{teal!20}0.126 ($\pm0.087$)$^\ddagger$\\\cline{2-9}
&&
  \texttt{\approach$_{ran}$}  &0.867 ($\pm0.006$)&0.859 ($\pm0.006$)&0.867 ($\pm0.013$)&0.868 ($\pm0.006$)&-52.139 ($\pm11.494$)&0.053 ($\pm0.002$)\\ 
&\multirow{-2}{*}{RoBERTa}&
  \texttt{\approach}  &\cellcolor{teal!20}0.875 ($\pm0.010$)$^\ddagger$&\cellcolor{teal!20}0.866 ($\pm0.010$)$^\ddagger$&\cellcolor{teal!20}0.882 ($\pm0.015$)$^\ddagger$&0.869 ($\pm0.008$)&\cellcolor{teal!20}-16.749 ($\pm24.792$)$^\ddagger$&\cellcolor{teal!20}0.137 ($\pm0.102$)$^\ddagger$\\\cline{2-9}
&&
  \texttt{\approach$_{ran}$} &0.881 ($\pm0.004$)&0.873 ($\pm0.004$)&0.887 ($\pm0.010$)&0.875 ($\pm0.007$)&-51.531 ($\pm9.335$)&0.053 ($\pm0.002$)\\
\multirow{-6}{*}{700} &\multirow{-2}{*}{RTA} &
  \texttt{\approach}  &\cellcolor{teal!20}0.885 ($\pm0.006$)$^\ddagger$&\cellcolor{teal!20}0.877 ($\pm0.006$)$^\ddagger$&\cellcolor{teal!20}0.894 ($\pm0.011$)$^\ddagger$&0.877 ($\pm0.006$)&\cellcolor{teal!20}-16.551 ($\pm21.921$)$^\ddagger$&\cellcolor{teal!20}0.139 ($\pm0.105$)$^\ddagger$\\\bottomrule

\end{tabular}
% }
\end{adjustbox}
\label{tab:rq3-1}
\end{table}%

==> tab/rq4.tex <==
\begin{table}[t!]
	\centering
        \footnotesize
	\setlength{\tabcolsep}{2mm}
	\caption{RQ4: Scott-Knott rank of metrics comparing~\approach with SOTA.. }
	\label{tab:rq1-1}%
	%\begin{threeparttable}
	\begin{tabular}{ccccccccc}\toprule
	\textbf{Step size}&\textbf{Methods/Metrics}\hspace{-0.5cm}&\textbf{F1-score}&\textbf{Accuracy}&\textbf{Recall}&\textbf{Precision}&\textbf{Readability}&\textbf{Identifiability}\\\midrule % times 27
  	
   \multirow{3}{*}{300} &Ours&1&1&2&1&1&1\\
   &Wu2021&5&5&1&5&3&2\\
   &Ge2021&2&2&5&2&2&2\\
   &Thung2015&3&3&3&4&4&3\\
   &Tu2022&4&4&4&3&5&4\\
\midrule
   \multirow{3}{*}{500} &Ours&1&1&2&1&1&1\\
   &Wu2021&5&5&1&5&3&2\\
   &Ge2021&2&2&5&2&2&2\\
   &Thung2015&3&3&3&4&4&3\\
   &Tu2022&4&4&4&3&5&4\\
\midrule
   \multirow{3}{*}{700} &Ours&1&1&2&1&1&1\\
   &Wu2021&5&5&1&5&3&2\\
   &Ge2021&2&2&5&2&2&2\\
   &Thung2015&3&3&3&4&4&3\\
   &Tu2022&4&4&4&3&5&4\\
	\end{tabular}	
\end{table}%

==> tab/rq4_avg.tex <==
% \begin{table}[t!]
% 	\centering
% 	\setlength{\tabcolsep}{2mm}
% 	\caption{RQ4: Average values of metrics comparing \approach with SOTA. The best value of each performance indicator is in \textcolor{red}{RED}.}
% 	\label{tab:rq4-1}%
% 	%\begin{threeparttable}
%     \footnotesize
% 	\begin{tabular}{ccccccccc}\toprule
% 	\textbf{Step size}&\textbf{Methods/Metrics}\hspace{-0.5cm}&\textbf{F1-score}&\textbf{Accuracy}&\textbf{Recall}&\textbf{Precision}&\textbf{Readability}&\textbf{Identifiability}\\\midrule % times 27

 
%     \multirow{5}{*}{300} &Ours&\textcolor{red}{0.871}&\textcolor{red}{0.862}&0.877&\textcolor{red}{0.866}&\textcolor{red}{-2.131}&\textcolor{red}{0.098}\\
%     &Wu2021&0.798&0.756&\textcolor{red}{0.905}&0.714&-82.204&0.052\\
%     &Ge2021&0.825&0.813&0.828&0.823&-79.678&0.052\\
%     &Thung2015&0.81&0.787&0.851&0.773&-83.085&0.052\\
%     &Tu2022&0.807&0.786&0.841&0.777&-91.182&0.049\\
% \midrule
%    \multirow{5}{*}{500}
%    &Ours&\textcolor{red}{0.878}&\textcolor{red}{0.869}&0.883&\textcolor{red}{0.873}&\textcolor{red}{-14.226}&\textcolor{red}{0.089}\\
%     &Wu2021&0.806&0.767&\textcolor{red}{0.909}&0.723&-82.328&0.052\\
%     &Ge2021&0.828&0.811&0.858&0.801&-79.38&0.052\\
%     &Thung2015&0.825&0.806&0.86&0.794&-78.149&0.052\\
%     &Tu2022&0.821&0.802&0.854&0.791&-87.323&0.053\\
% \midrule
%    \multirow{5}{*}{700}    &Ours&\textcolor{red}{0.880}&\textcolor{red}{0.871}&0.887&\textcolor{red}{0.873}&\textcolor{red}{-13.21}&\textcolor{red}{0.118}\\
%     &Wu2021&0.805&0.767&\textcolor{red}{0.905}&0.725&-90.846&0.049\\
%     &Ge2021&0.834&0.821&0.844&0.824&-90.171&0.049\\
%     &Thung2015&0.829&0.812&0.856&0.803&-89.226&0.05\\
%     &Tu2022&0.828&0.811&0.856&0.803&-92.546&0.051\\


%     \bottomrule
% 	\end{tabular}
% \end{table}%


\begin{table}[t!]
	\centering
	\setlength{\tabcolsep}{0.8mm}
	\caption{Comparing the mean and standard deviation (SD) of the metrics values for \approach~and the state-of-the-art approaches for bug report identification. The format is the same as Table~\ref{tab:rq1-1}.}
	\label{tab:rq4-1}%
% \resizebox{\textwidth}{!}{ % reSize the table
\begin{adjustbox}{width=\textwidth}
% \begin{tabular}{p{1cm}p{2cm}p{0.3cm}p{1.55cm}|p{0.3cm}p{1.55cm}|p{0.3cm}p{1.4cm}|p{0.3cm}p{1.4cm}|p{0.3cm}p{1.55cm}|p{0.3cm}p{1.4cm}}
\begin{tabular}{ll|llllllll|llllll}
\toprule
 \multirow{2}{*}{\textbf{Query Size}} &
  \multirow{2}{*}{\textbf{Approach}} &
  \multicolumn{2}{c}{\textbf{F1-score}} &
  \multicolumn{2}{c}{\textbf{Accuracy}} &
  \multicolumn{2}{c}{\textbf{Recall}} &
  \multicolumn{2}{c|}{\textbf{Precision}} &
  \multicolumn{2}{c}{\textbf{Readability}} &
  \multicolumn{2}{c}{\textbf{Identifiability}}\\ \cline{3-14}

 &
   &
  \textbf{$r$} &
  \textbf{Mean (SD)} &
  \textbf{$r$} &
  \textbf{Mean (SD)} &
  \textbf{$r$} &
  \textbf{Mean (SD)} &
  \textbf{$r$} &
  \textbf{Mean (SD)} &
  \textbf{$r$} &
  \textbf{Mean (SD)} &
  \textbf{$r$} &
  \textbf{Mean (SD)} \\ \midrule
%  &
%   \texttt{EMBLEM} &4&0.807&4&0.786&4&0.841&3&0.777&5&-91.182&4&0.049 \\
%  &
%   \texttt{hbrPredictor} &5&0.798&5&0.756&\cellcolor{teal!20}1&\cellcolor{teal!20}0.905&5&0.714&3&-82.204&2&0.052 \\
% &
%   Ge et al. &2&0.825&2&0.813&5&0.828&2&0.823&2&-79.678&2&0.052 \\   
% &
%   Thung et al. &3&0.81&3&0.787&3&0.851&4&0.773&4&-83.085&3&0.052\\
% \multirow{-5}{*}{300}  &
%   \approach  &\cellcolor{teal!20}1&\cellcolor{teal!20}0.87&\cellcolor{teal!20}1&\cellcolor{teal!20}0.861&2&0.872&\cellcolor{teal!20}1&\cellcolor{teal!20}0.868&\cellcolor{teal!20}1&\cellcolor{teal!20}6.779&\cellcolor{teal!20}1&\cellcolor{teal!20}0.115\\\hline
  
%  &
%   \texttt{EMBLEM} &4&0.821&4&0.802&4&0.854&3&0.791&5&-87.323&4&0.053 \\
%  &
%   \texttt{hbrPredictor} &5&0.806&5&0.767&\cellcolor{teal!20}1&\cellcolor{teal!20}0.909&5&0.723&3&-82.328&2&0.052 \\
% &
%   Ge et al. &2&0.828&2&0.811&5&0.858&2&0.801&2&-79.38&2&0.052 \\   
% &
%   Thung et al. &3&0.825&3&0.806&3&0.86&4&0.794&4&-78.149&3&0.052\\
% \multirow{-5}{*}{500}  &
%   \approach  &\cellcolor{teal!20}1&\cellcolor{teal!20}0.877&\cellcolor{teal!20}1&\cellcolor{teal!20}0.868&2&0.883&\cellcolor{teal!20}1&\cellcolor{teal!20}0.87&\cellcolor{teal!20}1&\cellcolor{teal!20}-8.392&\cellcolor{teal!20}1&\cellcolor{teal!20}0.09\\\hline
  
%  &
%   \texttt{EMBLEM} &4& 0.828&4&0.811&4&0.856&3&0.803&5&-92.546&4&0.051\\
%  &
%   \texttt{hbrPredictor} &5&0.805&5&0.767&1&\cellcolor{teal!20}0.905&5&0.725&3&-90.846&2&0.049 \\
% &
%   Ge et al. &2&0.834&2&0.821&5&0.844&2&0.824&2&-90.171&2&0.049 \\   
% &
%   Thung et al. &3&0.829&3&0.812&3&0.856&4&0.803&4&-89.226&3&0.05\\
% \multirow{-5}{*}{700}  &
%   \approach  &\cellcolor{teal!20}1&\cellcolor{teal!20}0.880&\cellcolor{teal!20}1&\cellcolor{teal!20}0.871&2&0.887&\cellcolor{teal!20}1&\cellcolor{teal!20}0.873&\cellcolor{teal!20}1&\cellcolor{teal!20}-10.246&\cellcolor{teal!20}1&\cellcolor{teal!20}0.094\\\bottomrule

 &
  \texttt{EMBLEM} &4&0.797 ($\pm0.011$)&4&0.775 ($\pm0.010$)&4&0.831 ($\pm0.025$)&3&0.767 ($\pm0.014$)&2&-87.015 ($\pm7.999$)&2&0.050 ($\pm0.002$)\\
 &
  \texttt{hbrPredictor} &4&0.796 ($\pm0.006$)&5&0.756 ($\pm0.005$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.894 ($\pm0.021$)&4&0.718 ($\pm0.009$)&2&-86.748 ($\pm13.417$)&2&0.050 ($\pm0.003$)\\
&
  Ge et al. &2&0.815 ($\pm0.013$)&2&0.803 ($\pm0.014$)&5&0.819 ($\pm0.031$)&2&0.813 ($\pm0.024$)&2&-86.625 ($\pm13.658$)&2&0.050 ($\pm0.003$)\\  
&
  Thung et al. &3&0.802 ($\pm0.009$)&3&0.778 ($\pm0.010$)&3&0.842 ($\pm0.021$)&3&0.766 ($\pm0.014$)&2&-86.505 ($\pm12.561$)&2&0.050 ($\pm0.002$)\\
\multirow{-5}{*}{300}  &
  \approach  &\cellcolor{teal!20}1&\cellcolor{teal!20}0.855 ($\pm0.018$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.847 ($\pm0.017$)&2&0.852 ($\pm0.031$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.859 ($\pm0.016$)&\cellcolor{teal!20}1&\cellcolor{teal!20}1.770 ($\pm36.207$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.167 ($\pm0.104$)\\\hline
  
 &
  \texttt{EMBLEM} &4&0.810 ($\pm0.009$)&4&0.789 ($\pm0.009$)&5&0.842 ($\pm0.015$)&4&0.779 ($\pm0.011$)&2&-88.767 ($\pm12.004$)&2&0.050 ($\pm0.001$)\\  
 &
  \texttt{hbrPredictor} &5&0.803 ($\pm0.003$)&5&0.764 ($\pm0.005$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.902 ($\pm0.011$)&5&0.724 ($\pm0.008$)&2&-87.837 ($\pm10.198$)&2&0.051 ($\pm0.002$)\\
&
  Ge et al. &2&0.823 ($\pm0.008$)&2&0.805 ($\pm0.010$)&3&0.853 ($\pm0.023$)&2&0.797 ($\pm0.021$)&2&-87.202 ($\pm10.415$)&2&0.050 ($\pm0.002$)\\
&
  Thung et al. &3&0.814 ($\pm0.009$)&3&0.794 ($\pm0.010$)&4&0.846 ($\pm0.018$)&3&0.784 ($\pm0.013$)&2&-87.023 ($\pm10.714$)&2&0.051 ($\pm0.002$)\\
\multirow{-5}{*}{500}  &
  \approach  &\cellcolor{teal!20}1&\cellcolor{teal!20}0.864 ($\pm0.015$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.856 ($\pm0.014$)&2&0.863 ($\pm0.026$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.865 ($\pm0.010$)&\cellcolor{teal!20}1&\cellcolor{teal!20}-2.511 ($\pm18.956$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.145 ($\pm0.106$)\\\hline
  
 &
  \texttt{EMBLEM} &4&0.819 ($\pm0.008$)&4&0.801 ($\pm0.009$)&4&0.844 ($\pm0.015$)&4&0.795 ($\pm0.009$)&2&-88.860 ($\pm9.759$)&2&0.051 ($\pm0.001$)\\
 &
  \texttt{hbrPredictor} &5&0.806 ($\pm0.003$)&5&0.770 ($\pm0.005$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.899 ($\pm0.010$)&5&0.731 ($\pm0.007$)&2&-88.194 ($\pm7.588$)&2&0.050 ($\pm0.001$)\\
&
  Ge et al. &2&0.829 ($\pm0.007$)&2&0.817 ($\pm0.006$)&5&0.835 ($\pm0.017$)&2&0.825 ($\pm0.010$)&2&-88.113 ($\pm7.541$)&2&0.050 ($\pm0.001$)\\
&
  Thung et al. &3&0.821 ($\pm0.008$)&3&0.804 ($\pm0.008$)&3&0.848 ($\pm0.015$)&3&0.797 ($\pm0.009$)&2&-88.102 ($\pm7.290$)&2&0.050 ($\pm0.001$)\\
\multirow{-5}{*}{700}  &
  \approach  &\cellcolor{teal!20}1&\cellcolor{teal!20}0.869 ($\pm0.011$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.861 ($\pm0.011$)&2&0.871 ($\pm0.019$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.868 ($\pm0.009$)&\cellcolor{teal!20}1&\cellcolor{teal!20}-10.555 ($\pm18.465$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.132 ($\pm0.100$)\\\bottomrule

\end{tabular}
\end{adjustbox}
% }
\end{table}%



==> tab/rq4_med.tex <==
\begin{table}[t!]
	\centering
	\setlength{\tabcolsep}{2mm}
	\caption{RQ4: Median values of metrics comparing \approach with SOTA. The best value of each performance indicator is in \textcolor{red}{RED}.}
	\label{tab:rq4-1}%
	%\begin{threeparttable}
    \footnotesize
	\begin{tabular}{ccccccccc}\toprule
	\textbf{Step size}&\textbf{Methods/Metrics}\hspace{-0.5cm}&\textbf{F1-score}&\textbf{Accuracy}&\textbf{AUC}&\textbf{Recall}&\textbf{Precision}&\textbf{Readability}&\textbf{Identifiability}\\\midrule % times 27

 
    \multirow{5}{*}{300} 
    &Ours&\textcolor{red}{0.872}&\textcolor{red}{0.862}&\textcolor{red}{0.918}&0.877&\textcolor{red}{0.865}&\textcolor{red}{-3.491}&\textcolor{red}{0.098}\\
    &Wu2021&0.797&0.755&0.745&\textcolor{red}{0.909}&0.714&-82.543&0.052\\
    &Ge2021&0.825&0.814&0.813&0.827&0.824&-78.861&0.052\\
    &Thung2015&0.809&0.785&0.781&0.852&0.77&-82.436&0.052\\
    &Tu2022&0.805&0.786&0.783&0.839&0.777&-87.992&0.049\\
\midrule
   \multirow{5}{*}{500}
   &Ours&\textcolor{red}{0.878}&\textcolor{red}{0.87}&\textcolor{red}{0.916}&0.883&\textcolor{red}{0.872}&\textcolor{red}{-14.705}&\textcolor{red}{0.089}\\
    &Wu2021&0.806&0.767&0.757&\textcolor{red}{0.909}&0.724&-81.647&0.052\\
    &Ge2021&0.829&0.812&0.809&0.86&0.802&-78.976&0.052\\
    &Thung2015&0.825&0.807&0.803&0.86&0.795&-77.563&0.052\\
    &Tu2022&0.821&0.801&0.798&0.852&0.792&-88.342&0.053\\
\midrule
   \multirow{5}{*}{700}    
   &Ours&\textcolor{red}{0.879}&\textcolor{red}{0.87}&\textcolor{red}{0.919}&0.886&\textcolor{red}{0.873}&\textcolor{red}{-12.524}&\textcolor{red}{0.094}\\
    &Wu2021&0.805&0.766&0.756&\textcolor{red}{0.906}&0.724&-89.764&0.049\\
    &Ge2021&0.834&0.82&0.818&0.844&0.823&-89.183&0.049\\
    &Thung2015&0.829&0.812&0.809&0.857&0.805&-88.9&0.05\\
    &Tu2022&0.828&0.811&0.808&0.856&0.803&-92.466&0.051\\


    \bottomrule
	\end{tabular}
\end{table}%

==> tab/rq5.tex <==
% \begin{table}[t!]
% 	\centering
% 	%\setlength{\tabcolsep}{2mm}
% 	\caption{Comparing \approach~and \approach$_{ran}$ in the qualitative study. The best is highlighted in \setlength{\fboxsep}{1.5pt}\colorbox{teal!20}{green}.}
% 	\label{tab:rq5-1}%
% 	%\begin{threeparttable}
%     % \footnotesize
%     \begin{adjustbox}{width=\textwidth}
% 	\begin{tabular}{llllll}\toprule
% 	\textbf{Type}&\textbf{Metric}&\textbf{\approach$_{ran}$}&\textbf{\approach}&\textbf{$p$-value}&\textbf{$\hat{A}_{12}$}\\\midrule % times 27

%    \multirow{2}{*}{Effort} &Mean/deviation of readability score&0.79 ($\pm 0.83$)&\cellcolor{teal!20}0.20 ($\pm 0.47$)&$6.27 \times 10^-21$&0.872\\
%    &Mean/deviation of identifiability score&0.71 ($\pm 0.88$)&\cellcolor{teal!20}0.25 ($\pm 0.48$)&$2.00 \times 10^-13$&0.652\\
% \hline
%     \multirow{2}{*}{Time} &Total labeling time for a timestep (300 reports)&128 mins&\cellcolor{teal!20}40 mins&-&-\\
%     &Expected number of reports labeled per hour&140&\cellcolor{teal!20}460&-&-\\
% \hline
%     \multirow{1}{*}{Money} &Total monetary cost for labeling in a timestep (300 reports)&\pounds21.91&\cellcolor{teal!20}\pounds6.67&-&-\\
%     % &Expected money cost for 10 steps&\pounds219.11&\textcolor{red}{\pounds66.74}\\
% %&2.14 hours&\textcolor{red}{0.65 hours}\\
%     \bottomrule
% 	\end{tabular}
%  \end{adjustbox}
% \end{table}%

\begin{table}[t!]
	\centering
	%\setlength{\tabcolsep}{2mm}
	\caption{Comparing \approach~and \approach$_{ran}$ in the qualitative study involving humans. The format is the same as Table~\ref{tab:rq2-1}.}
	\label{tab:rq5-1}%
	%\begin{threeparttable}
    % \footnotesize
    \begin{adjustbox}{width=0.8\textwidth}
	\begin{tabular}{llllll}\toprule
	\textbf{Type}&\textbf{Metric}&\textbf{\approach$_{ran}$}&\textbf{\approach}\\\midrule % times 27

   \multirow{2}{*}{Effort} &Mean/deviation of readability score&0.79 ($\pm 0.83$)&\cellcolor{teal!20}0.20 ($\pm 0.47$)$^\ddagger$\\
   &Mean/deviation of identifiability score&0.71 ($\pm 0.88$)&\cellcolor{teal!20}0.25 ($\pm 0.48$)$^\ddagger$\\
\hline
    \multirow{2}{*}{Time} &Total labeling time for a timestep (300 reports)&128 mins&\cellcolor{teal!20}40 mins\\
    &Expected number of reports labeled per hour&140&\cellcolor{teal!20}460\\
\hline
    \multirow{1}{*}{Money} &Total monetary cost for labeling in a timestep (300 reports)&\pounds21.91&\cellcolor{teal!20}\pounds6.67\\
    % &Expected money cost for 10 steps&\pounds219.11&\textcolor{red}{\pounds66.74}\\
%&2.14 hours&\textcolor{red}{0.65 hours}\\
    \bottomrule
	\end{tabular}
 \end{adjustbox}
\end{table}%

==> tab/sota.tex <==

\begin{table}
% \footnotesize
  \caption{The state-of-the-art active learning approaches for bug report identification or a similar problem. (TF-IDF, NBM, RF, and SVM stand for Term Frequency–Inverse Document Frequency, Multinomial Naive Bayes, Random Forest, and Support Vector Machine, respectively.)}
  \label{tab:sota}
  \begin{adjustbox}{width=0.8\textwidth}
  % \footnotesize
      % \setlength{\tabcolsep}{1mm}
%\begin{threeparttable}
  \begin{tabular}{lllll}
    \toprule
    \textbf{Name}&\textbf{Model}&\textbf{Sampling}&\textbf{Pseudo Labeling}&\textbf{Year}\\
    \midrule


\citeauthor{DBLP:conf/iwpc/ThungLL15}~\cite{DBLP:conf/iwpc/ThungLL15}&TF-IDF and SVM&Uncertainty&No&2015\\

    \texttt{hbrPredictor}~\cite{DBLP:journals/infsof/WuZCZYM21}&TF-IDF and NBM&Uncertainty&No&2021\\

    \citeauthor{DBLP:journals/infsof/GeFQGQ22}~\cite{DBLP:journals/infsof/GeFQGQ22}&TF-IDF and RF&Uncertainty&No&2021\\

    

    \texttt{EMBLEM}~\cite{DBLP:journals/tse/TuYM22}&TF-IDF and SVM&Uncertainty and Certainty&No&2022\\
    %TF-IDF/NBM&Uncertainty&hbrPredictor&\citeauthor{DBLP:journals/infsof/WuZCZYM21}~\cite{DBLP:journals/infsof/WuZCZYM21}&2021\\

   % TF-IDF/RF&Uncertainty&Ge2021&\citeauthor{DBLP:journals/infsof/GeFQGQ22}~\cite{DBLP:journals/infsof/GeFQGQ22}&2021 \\

    %TF-IDF/SVM&Uncertainty&Thung2015&\citeauthor{DBLP:conf/iwpc/ThungLL15}~\cite{DBLP:conf/iwpc/ThungLL15}&2015  \\

    %TF-IDF/SVM&Uncertainty+Certainty&EMBLEM&\citeauthor{DBLP:journals/tse/TuYM22}~\cite{DBLP:journals/tse/TuYM22}&2022 \\

  \bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

==> tab/test.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table*}[t!]
% \footnotesize
% \setlength{\tabcolsep}{1mm}
% \renewcommand\arraystretch{1.3}
\resizebox{\textwidth}{!}{ % reSize the table
\begin{tabular}{p{0.7cm}p{2cm}p{0.3cm}p{1.55cm}|p{0.3cm}p{1.55cm}|p{0.3cm}p{1.4cm}|p{0.3cm}p{1.4cm}|p{0.3cm}p{1.55cm}|p{0.3cm}p{1.4cm}}
\toprule
 &
  \multirow{2}{*}{\textbf{Approach}} &
  \multicolumn{2}{c}{\textsc{\textbf{F1-score}}} &
  \multicolumn{2}{c}{\textsc{\textbf{Accuracy}}} &
  \multicolumn{2}{c}{\textsc{\textbf{Recall}}} &
  \multicolumn{2}{c}{\textsc{\textbf{Precision}}} &
  \multicolumn{2}{c}{\textsc{\textbf{Readability}}} &
  \multicolumn{2}{c}{\textsc{\textbf{Identifiability}}}\\ \cline{3-14}

 &
   &
  \textbf{$r$} &
  \textbf{Med (IQR)} &
  \textbf{$r$} &
  \textbf{Med (IQR)} &
  \textbf{$r$} &
  \textbf{Med (IQR)} &
  \textbf{$r$} &
  \textbf{Med (IQR)} &
  \textbf{$r$} &
  \textbf{Med (IQR)} &
  \textbf{$r$} &
  \textbf{Med (IQR)} & \\ \hline
 &
  \texttt{Random}  &1&1&1&1&1&1&1&1&1&1&1&1\\
 &
  \texttt{Uncertainty} &1&1&1&1&1&1&1&1&1&1&1&1 \\
\multirow{-3}{*}{300} &
  \texttt{Effort} &1&1&1&1&1&1&1&1&1&1&1&1 \\  \hline
  
 &
  \texttt{Random}  &1&1&1&1&1&1&1&1&1&1&1&1\\
 &
  \texttt{Uncertainty} &1&1&1&1&1&1&1&1&1&1&1&1 \\
\multirow{-3}{*}{500} &
  \texttt{Effort} &1&1&1&1&1&1&1&1&1&1&1&1 \\  \hline
  
 &
  \texttt{Random}  &1&1&1&1&1&1&1&1&1&1&1&1\\
 &
  \texttt{Uncertainty} &1&1&1&1&1&1&1&1&1&1&1&1 \\
\multirow{-3}{*}{700} &
  \texttt{Effort} &1&1&1&1&1&1&1&1&1&1&1&1 \\ 

 
\bottomrule
\end{tabular}
}
% \end{table*}

